Exploring Long Tail Visual Relationship Recognition with Large Vocabulary

Several approaches have been proposed in recent literature to alleviate the long-tail problem, mainly in object classification tasks. In this paper, we make the first large-scale study concerning the task of Long-Tail Visual Relationship Recognition (LTVRR). LTVRR aims at improving the learning of structured visual relationships that come from the long-tail (e.g., "rabbit grazing on grass"). In this setup, the subject, relation, and object classes each follow a long-tail distribution. To begin our study and make a future benchmark for the community, we introduce two LTVRR-related benchmarks, dubbed VG8K-LT and GQA-LT, built upon the widely used Visual Genome and GQA datasets. We use these benchmarks to study the performance of several state-of-the-art long-tail models on the LTVRR setup. Lastly, we propose a visiolinguistic hubless (VilHub) loss and a Mixup augmentation technique adapted to LTVRR setup, dubbed as RelMix. Both VilHub and RelMix can be easily integrated on top of existing models and despite being simple, our results show that they can remarkably improve the performance, especially on tail classes. Benchmarks, code, and models have been made available at: https://github.com/Vision-CAIR/LTVRR.

==> LaTeX/analysis.tex <==


\subsection{Word2vec/Embeddings Analysis Protocol.}

\begin{figure}[ht!]
\centering
 \includegraphics[width=0.5\textwidth]{figures/motivation_metric.png}
  \caption{Gold has good precision (not shown), but poor recall (left panel).Motivation for our proposed analysis validated by 3 high-quality Human Subjects Experiments on 100 visual relationships. On the left, the x axis the rank by the prediction by~\cite{zhang2019large} and y axis is the recall of predictions that are good or better (3 human subjects (\textcolor{mygray}{gray}, \textcolor{blue}{blue}, \textcolor{red}{red}) and the \textcolor{gold_web}{\textbf{gold}} as the ground truth). On the right, votes  rank by 3 Human Subjects with each score from 1 to 5(best seen in color). Black is the real distribution and the red is the corresponding Poisson point process. }
\label{fig:humansbj_exp}
\end{figure}

\begin{figure}[ht!]
\centering
 \includegraphics[width=0.3\textwidth]{figures/motivation_metric_example.png}
  \caption{This example is meant to show how some boxes can have multiple good answers. The top 5 predictions for the above box ares: [Baseball Cap, Cap, Green Hat, Hat, Head]. This shows how it is unreasonable to evaluate this task assuming there is only one correct answer.}
\label{fig:metric_motive_exp}
\end{figure}


\begin{figure}[hb!]
\centering
 \includegraphics[width=0.5\textwidth]{{figures/analysis_tool.png}
 \caption{Word2Vec_V is systematically better than the alternatives as observed in the figure above showing an analysis of Six Word2vec (LCH    WUP    RES    JCN    LIN    PATH),  two word embedding metrics (Visual word2vec and Language Word2vec) on the approach of~\cite{zhang2019large} in comparison with the standard exact match accuracy (ACC).}
\label{fig_analysis_word2vec}
\end{figure}



Fig~\ref{fig:humansbj_exp} shows a human subject experiment that motivates an analysis methodology that we propose here to analyze different methods based on WordNet and word2vec.  We chose randomly 100 visual relationship validation examples and evaluated 5 hypotheses for each; Ground Truth (GT) and the top 4 predictions by~\cite{zhang2019large} excluding GT. Hence, we collected a total of 500  responses from human subjects ranging from 1 (awful) to 5 (excellent).  We tried both Mechanical Turk~\cite{buhrmester2011amazon} and graduate students in the  AI field and we observed better consistency and inter-rater agreement within  AI researchers,  measured with Cohen's Kappa score~\cite{cohen1960coefficient}, and hence we focus on them here\footnote{The inner annotator analysis for AI researchers vs Turkers can be found in the supplementary}. Fig~\ref{fig:humansbj_exp} (on the left) shows responses of 3 human subjects (\textcolor{mygray}{gray}, \textcolor{blue}{blue}, \textcolor{red}{red}) whose responses ranges from 1 to 5 (excellent). We additionally regard the ground truth with ~\textcolor{gold_web}{\textbf{gold}} color as a binary judge where only one of the five is 5 (excellent) and rest is 0. We also binarize all scores to be correct if the score is $\ge 3$ (good) and not correct otherwise. We show on the left of the figure the recall of each one of the subjects and the ground truth judged by the majority vote of the remaining three. This shows how the human subjects are in agreement that the system is still capable of producing reasonable answers in the top 4 ranks going from left to right. In the meantime,  the ground truth is missing that as reflected in the low recall especially and it gets more severe as we move to the lower ranks.  Fig~\ref{fig:humansbj_exp} (on the right), we show the distribution from 3 to 15 summing up scores of 4 subjects each ranging from 1 to 5. The curve illustrates that the real distribution tends to be closer toward the satisfactory spectrum ($>10$). This observation also motivates us to propose a metric that helps alleviate this missing evaluation perspective that we reflect on in our experiments. %\textcolor{blue}{ in both the head and the tail analysis. VISIT after the analysis is done. }

The main motivation behind proposing these metrics is that this task does not have a single correct answer. There are many examples where there is more than one reasonable answer. The human judges confirm that, but the gold doesn't allow for that (by construction). The construction assumes that there is one and only one right answer. Fig~\ref{fig:metric_motive_exp} shows an example of such case. In this case, the top 5 predictions from the model are all correct and very plausible. It's very hard to say any of these are wrong. This illustrates that the gold standard with one correct answer only is fundamentally flawed for this task, and this is the motivation behind our proposed metrics.

\noindent \textbf{Proposed WordNet/Word Embedding Analysis protocol.} Given that there are often multiple good answers, can we come up with some kind of soft matching method to give partial credit to answers that aren't in the gold but are close? Motivated by the former human study, we propose to perform analysis based on six wordnet~\cite{miller1995wordnet} metrics that have been investigated/ used in the literature (Leacock-Chodorow Similarity(LCH),  Wu-Palmer Similarity(WUP), Resnik (RES), and path similarity (PATH)~\footnote{reference to the implementation we used of these six functions  \url{http://www.nltk.org/howto/wordnet.html}}, and two visual and language word embedding we discussed in Sec.~\ref{sec_approach}. For each test example, we start by producing the top 250 closest predictions and store the corresponding confidence. Then, we use each of these metrics to retrieve the top $T$ closest labels in the list of 250 predicted labels according to the chosen metric and mark it as relevant (label 1) to the test example in addition to the ground truth. We mark the remaining labels as irrelevant  (label 0). After that, we report the Average Precision(AP) at 1, 5, 20, and 50 on the system. What this analysis tool measure is the capability of the system to bring concepts that are related to the ground truth according to the given language metric up in the rank.   



In fig.~\ref{fig_analysis_word2vec}, we show using this analysis protocol on the baseline state of the art approach  by~\cite{zhang2019large}. The figures show the AP@1, AP@5, AP@10, and AP@5 using all 8 metrics on the y Axis. The figure shows the Visual word2vec makes the system look the best compared to all the other metrics including the language word2vec and the six wordNet metrics. This is since the system was word embeddings as input during training. In our remaining experiments, we show  that other wordNet based analysis is still useful as an analysis tool since other approaches can be evaluated on their skill to bring relevant concepts according to WordNet-based metrics up in the rank.  In  fig.~\ref{fig_analysis_word2vec}, visual word2vec is 13.0\% and 23.07\% better than language word2vec on AP@1 and AP@50 respectively.  In this analysis, each example whether it is in the head or the tail contributes equally, and hence the results in this section is more dominated by the head as it contributes with many more examples. We show later that this analysis can be adapted to let all head and tail classes contribute equally under this metric. After adapting this metric to long-tail, we realized that this system looks better in language word2vec versus visual word2vec; discussed later in  Table 2. We find this interesting as it means that Visual Word embeddings are more useful to head the classes, while language word embeddings are more beneficial to tail classes.
 







==> LaTeX/discussions.tex <==
We summarize the main observations from our experiments as follows:\\
1. Adding the ViL-Hubless loss almost always improves the performance on tail classes; both for standard recognition (classifying subject as \textit{man}) and for the more complex case of recognizing a relation between two interacting objects.\\
2. The standard evaluation metrics that are commonly used are missing some aspects, since ground truth annotations are incomplete especially for large-scale long-tail problems like ours. Hence, our new analysis measures can augment the evaluation, offering an additional intuitive  view on how the models are performing.\\
%Based on the observations we offer our answers to some of the questions that may arise to the readers.
% In this section we offer our answers to some of the questions that may arise to the readers.
\textit{ \textbf{What's new about this task?} } Existing literature on visual relationship understanding  covers studying rare combinations of S, R, and O, while each of S, R, and O has a sufficient number of examples (i.e. head). In LTVRR, each of the S, R, and O distributions follow a  long-tail distribution.\\ %In addition to that, we use the raw distributions from the datasets without doing any filtering based on frequency. This brings this visual understanding problem closer to real and more challenging world distribution.
%Yet, it is much more challenging.
\textit{\textbf{What is the purpose of using the ViLHub loss?}} The ViLHub loss acts as a regularizer for the models to prevent the model from ignoring the tail and encourages the system to be more predictive of  the tail.
 The goal here is \textit{\textbf{not} } to show that the ViLHub loss should be used as an alternative to other SOTA methods, but to show that the ViLHub loss is orthogonal and can be integrated with several methods  offering long-tail  performance benefits, especially on tail classes.\\
\textit{\textbf{What is the point of the new analysis measures?}} The long-tail problem offers unique challenges due to the sheer number of classes involved. The standard evaluation metrics can be too harsh for the long-tail problem. We introduce these analysis measures as a tool that can give  a deeper insight into how the models are performing.\\
\textit{\textbf{Does Long-Tail Structured Visual Understanding relate to / benefit other tasks ?}} We believe that structured visio-linguistic understanding is important as we have shown here in the context of Visual Relationship Recognition. However, structured visual understanding is inherently related to a variety of compositional tasks; e.g., it manifests itself on the spatial relations between 3D objects placed in real-world scenes \cite{achlioptas2020referit3d}, or in the part-based composition of common objects \cite{PartModels2010,Dubrovina_2019_ICCV}. It could be thus interesting to investigate how we can improve generalization on the tail by combining problem-dependent meta-information (structure), with the problem-agnostic ViLHub loss, Focal loss, or Equalization loss.

==> tables/experimental_tables.tex <==
\begin{table*}
GQA

\begin{tabular}{lrrrrrrrr}
\toprule
{} &  many\_s &  medium\_s &  few\_s &  all\_s &  many\_r &  medium\_r &  few\_r &  all\_r \\
\midrule
baseline       &    70.5 &      36.2 &    3.5 &   51.9 &    50.7 &       5.5 &    0.2 &   49.7 \\
hub            &    70.4 &      37.0 &    3.5 &   52.0 &    50.7 &       4.9 &    0.1 &   49.7 \\
hub1k          &    70.5 &      36.4 &    3.5 &   51.9 &    50.2 &       6.9 &    0.0 &   49.2 \\
hub5k          &    70.3 &      37.8 &    4.2 &   52.3 &    49.6 &       9.2 &    0.3 &   48.7 \\
hub10k         &    70.3 &      38.7 &    4.9 &   52.7 &    49.8 &       9.5 &    0.3 &   48.9 \\
hub20k         &    70.2 &      39.9 &    6.0 &   53.1 &    49.5 &       9.3 &    0.2 &   48.6 \\
hub50k         &    69.8 &      41.4 &    7.6 &   53.5 &    49.0 &       8.4 &    0.2 &   48.1 \\
hub100k        &    69.9 &      41.9 &    8.8 &   53.8 &    48.8 &       7.2 &    0.1 &   47.9 \\
hub500k        &    69.8 &      42.1 &    9.5 &   53.9 &    47.9 &       3.6 &    0.1 &   46.9 \\
focal\_5        &    69.6 &      38.0 &    4.7 &   52.1 &    50.5 &       6.0 &    0.1 &   49.6 \\
focal\_5\_hub20k &    69.8 &      41.7 &    8.1 &   53.7 &    49.0 &       7.0 &    0.1 &   48.1 \\
w\_ce           &    39.3 &      36.5 &   16.2 &   35.5 &    35.9 &      29.0 &   14.3 &   35.6 \\
w\_ce\_hub20k    &    35.2 &      39.5 &   18.8 &   34.2 &    33.5 &      31.3 &   15.6 &   33.3 \\
fc             &    71.6 &      26.9 &    0.1 &   49.5 &    50.0 &       0.0 &    0.0 &   49.0 \\
fc\_hub100k     &    71.4 &      32.5 &    0.4 &   51.0 &    49.5 &       0.0 &    0.0 &   48.5 \\
dcpl\_t01       &    71.4 &      27.0 &    0.1 &   49.4 &    50.0 &       0.0 &    0.0 &   48.9 \\
dcpl           &    61.0 &      34.1 &    4.4 &   45.9 &    46.7 &      17.9 &    0.4 &   46.0 \\
dcpl\_hub100k   &    58.2 &      38.2 &    6.3 &   45.7 &    40.4 &      21.0 &    0.9 &   39.9 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrr}
\toprule
{} &  many\_s\_pc &  medium\_s\_pc &  few\_s\_pc &  many\_r\_pc &  medium\_r\_pc &  few\_r\_pc &  all\_s\_pc &  all\_r\_pc \\
\midrule
baseline       &       64.2 &         29.6 &       1.0 &       43.0 &          5.1 &       0.1 &       8.5 &       3.0 \\
hub            &       64.1 &         30.4 &       1.0 &       42.8 &          4.9 &       0.0 &       8.6 &       3.0 \\
hub1k          &       64.2 &         29.8 &       1.0 &       45.3 &          6.2 &       0.0 &       8.5 &       3.3 \\
hub5k          &       64.4 &         31.4 &       1.2 &       46.0 &          7.3 &       0.2 &       8.9 &       3.7 \\
hub10k         &       64.7 &         32.4 &       1.5 &       46.2 &          7.2 &       0.2 &       9.3 &       3.6 \\
hub20k         &       64.8 &         33.7 &       1.9 &       46.3 &          6.6 &       0.1 &       9.8 &       3.5 \\
hub50k         &       64.7 &         35.8 &       2.6 &       46.3 &          5.5 &       0.1 &      10.7 &       3.3 \\
hub100k        &       64.7 &         36.6 &       3.1 &       46.4 &          4.7 &       0.1 &      11.2 &       3.2 \\
hub500k        &       64.3 &         36.8 &       3.5 &       46.0 &          2.3 &       0.1 &      11.5 &       2.8 \\
focal\_5        &       64.1 &         31.8 &       1.4 &       40.3 &          5.4 &       0.0 &       9.1 &       2.9 \\
focal\_5\_hub20k &       64.7 &         36.2 &       2.8 &       46.0 &          4.4 &       0.1 &      10.9 &       3.1 \\
w\_ce           &       45.2 &         34.2 &       8.0 &       38.9 &         29.5 &       8.2 &      13.8 &      13.0 \\
w\_ce\_hub20k    &       43.1 &         37.2 &       9.8 &       39.1 &         32.8 &       8.4 &      15.6 &      13.6 \\
fc             &       64.5 &         19.1 &       0.0 &       29.8 &          0.0 &       0.0 &       6.1 &       1.5 \\
fc\_hub100k     &       65.7 &         24.1 &       0.1 &       36.2 &          0.0 &       0.0 &       7.0 &       1.9 \\
dcpl\_t01       &       63.8 &         19.3 &       0.0 &       29.1 &          0.0 &       0.0 &       6.1 &       1.5 \\
dcpl           &       60.1 &         28.2 &       1.2 &       45.9 &         15.3 &       0.1 &       8.2 &       4.7 \\
dcpl\_hub100k   &       59.6 &         32.5 &       1.9 &       45.4 &         17.9 &       0.2 &       9.4 &       5.2 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &  o\_s\_acc &  o\_s\_mr &  o\_r\_acc &  o\_r\_mr &  o\_t\_acc &  p\_s\_acc &  p\_s\_mr &  p\_r\_acc &  p\_r\_mr &  p\_t\_r\_acc &  p\_t\_s\_acc \\
\midrule
baseline       &     51.9 &    14.6 &     49.7 &     1.0 &     14.7 &      8.5 &   165.8 &      3.0 &    72.2 &        1.1 &        2.3 \\
hub            &     52.1 &    14.8 &     49.7 &     1.0 &     14.8 &      8.6 &   168.2 &      3.0 &    73.2 &        1.1 &        2.3 \\
hub1k          &     52.0 &    14.7 &     49.2 &     1.2 &     14.6 &      8.5 &   166.7 &      3.3 &    71.3 &        1.2 &        2.2 \\
hub5k          &     52.4 &    14.3 &     48.7 &     2.3 &     14.6 &      8.9 &   161.1 &      3.7 &    76.1 &        1.3 &        2.4 \\
hub10k         &     52.8 &    14.0 &     48.9 &     3.0 &     14.9 &      9.3 &   156.1 &      3.6 &    76.0 &        1.2 &        2.5 \\
hub20k         &     53.2 &    13.6 &     48.6 &     3.9 &     15.0 &      9.8 &   149.6 &      3.5 &    75.8 &        1.2 &        2.6 \\
hub50k         &     53.6 &    13.0 &     48.1 &     5.3 &     15.2 &     10.7 &   136.2 &      3.3 &    77.3 &        1.2 &        2.9 \\
hub100k        &     53.9 &    12.9 &     47.9 &     6.6 &     15.3 &     11.2 &   125.3 &      3.2 &    77.3 &        1.2 &        3.0 \\
hub500k        &     54.0 &    16.1 &     46.9 &     9.8 &     15.1 &     11.6 &   117.3 &      2.8 &    82.0 &        1.0 &        3.1 \\
focal\_5        &     52.1 &    14.8 &     49.6 &     1.1 &     14.7 &      9.1 &   170.5 &      2.9 &    73.3 &        1.1 &        2.4 \\
focal\_5\_hub20k &     53.8 &    13.6 &     48.1 &     5.1 &     15.3 &     11.0 &   144.3 &      3.1 &    80.4 &        1.2 &        3.0 \\
w\_ce           &     35.8 &    22.7 &     35.6 &     2.7 &      5.3 &     13.9 &    80.9 &     13.0 &    40.2 &        2.5 &        1.9 \\
w\_ce\_hub20k    &     34.6 &    20.6 &     33.3 &     5.2 &      4.7 &     15.7 &    73.2 &     13.6 &    39.6 &        2.5 &        1.9 \\
fc             &     49.4 &    47.7 &     49.0 &     1.7 &     13.4 &      6.1 &   604.6 &      1.5 &   141.6 &        0.5 &        1.6 \\
fc\_hub100k     &     51.0 &    43.7 &     48.5 &     6.4 &     14.0 &      7.0 &   586.7 &      1.9 &   127.2 &        0.6 &        1.8 \\
dcpl\_t01       &     49.3 &    48.1 &     48.9 &     1.7 &     13.3 &      6.1 &   606.6 &      1.5 &   141.1 &        0.5 &        1.6 \\
dcpl           &     45.9 &    25.8 &     46.0 &     1.4 &     11.1 &      8.2 &   355.0 &      4.7 &   108.3 &        1.3 &        1.9 \\
dcpl\_hub100k   &     45.8 &    24.3 &     39.9 &     3.7 &      9.5 &      9.4 &   334.3 &      5.2 &    66.6 &        1.5 &        1.9 \\
\bottomrule
\end{tabular}
\end{table*}

\newpage

VG
\begin{table*}
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  many\_s &  medium\_s &  few\_s &  all\_s &  many\_r &  medium\_r &  few\_r &  all\_r \\
\midrule
baseline    &    65.5 &      16.6 &    0.3 &   46.8 &    58.9 &       1.8 &    0.0 &   54.0 \\
hub10k      &    66.2 &      18.4 &    0.4 &   47.6 &    57.6 &       2.0 &    0.0 &   52.8 \\
hub100k     &    65.7 &      24.2 &    1.3 &   48.4 &    56.0 &       0.2 &    0.0 &   51.3 \\
w\_ce        &    46.7 &      29.7 &    5.4 &   37.3 &    25.1 &      16.7 &    3.3 &   23.8 \\
w\_ce\_hub20k &    44.3 &      30.3 &    6.1 &   36.0 &    24.6 &      16.5 &    3.3 &   23.4 \\
focal\_5     &    59.8 &      22.7 &    0.8 &   44.2 &    54.9 &       1.1 &    0.0 &   50.3 \\
fc          &    68.1 &      13.2 &    0.0 &   43.1 &    57.7 &       0.0 &    0.0 &   51.3 \\
dcpl        &    60.9 &       9.6 &    0.0 &   42.4 &    46.4 &       2.3 &    0.0 &   42.6 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrr}
\toprule
{} &  many\_s\_pc &  medium\_s\_pc &  few\_s\_pc &  many\_r\_pc &  medium\_r\_pc &  few\_r\_pc &  all\_s\_pc &  all\_r\_pc \\
\midrule
baseline    &       56.6 &         11.7 &       0.1 &       12.8 &          0.9 &       0.0 &       4.1 &       0.7 \\
hub10k      &       57.9 &         13.2 &       0.1 &       16.2 &          1.0 &       0.0 &       4.3 &       0.9 \\
hub100k     &       59.8 &         18.6 &       0.4 &       16.4 &          0.1 &       0.0 &       5.2 &       0.8 \\
w\_ce        &       51.4 &         25.4 &       2.5 &       26.6 &         13.5 &       1.6 &       7.3 &       4.1 \\
w\_ce\_hub20k &       50.6 &         26.3 &       3.0 &       26.8 &         13.5 &       1.4 &       7.7 &       3.9 \\
focal\_5     &       56.7 &         15.9 &       0.2 &       13.0 &          0.5 &       0.0 &       4.6 &       0.7 \\
fc          &       60.3 &          8.3 &       0.0 &        9.5 &          0.0 &       0.0 &       3.9 &       0.5 \\
dcpl        &       52.0 &          6.0 &       0.0 &       23.7 &          1.4 &       0.0 &       3.2 &       1.3 \\
\bottomrule
\end{tabular}


\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &  o\_s\_acc &  o\_s\_mr &  o\_r\_acc &  o\_r\_mr &  o\_t\_acc &  p\_s\_acc &  p\_s\_mr &  p\_r\_acc &  p\_r\_mr &  p\_t\_r\_acc &  p\_t\_s\_acc \\
\midrule
baseline    &     47.4 &    53.6 &     54.0 &    20.5 &     14.2 &      4.1 &   502.7 &      0.7 &   414.1 &        0.2 &        1.2 \\
hub10k      &     48.2 &    53.7 &     52.8 &    22.0 &     14.5 &      4.4 &   502.0 &      0.9 &   417.5 &        0.3 &        1.3 \\
hub100k     &     49.5 &    49.0 &     51.3 &    34.4 &     15.4 &      5.4 &   455.0 &      0.8 &   445.6 &        0.3 &        1.6 \\
w\_ce        &     40.0 &    47.6 &     23.8 &    29.9 &      5.3 &      7.5 &   238.0 &      4.1 &   250.9 &        0.7 &        0.7 \\
w\_ce\_hub20k &     38.8 &    49.0 &     23.4 &    29.4 &      5.0 &      7.9 &   228.5 &      3.9 &   235.7 &        0.7 &        0.8 \\
focal\_5     &     45.3 &    62.3 &     50.3 &    25.4 &     12.0 &      4.7 &   575.3 &      0.7 &   475.4 &        0.2 &        1.2 \\
fc          &     44.5 &   171.2 &     51.3 &    37.0 &     11.0 &      4.1 &  1334.1 &      0.5 &   660.0 &        0.1 &        1.0 \\
dcpl        &     43.1 &   128.0 &     42.6 &    30.5 &      9.5 &      3.3 &  1308.3 &      1.3 &   710.8 &        0.3 &        0.6 \\
\bottomrule
\end{tabular}


\end{table*}


==> tables/fine-grained/gvqa_per_class_mean_analysis.tex <==
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top1 &       {\bf 2.3} \\
 focal\_loss\_g025 &             rel &   top1 &     1.8 \\
   focal\_loss\_g1 &             rel &   top1 &     1.8 \\
  focal\_loss\_g10 &             rel &   top1 &     2.0 \\
   focal\_loss\_g2 &             rel &   top1 &     1.8 \\
   focal\_loss\_g5 &             rel &   top1 &     1.9 \\
  focal\_loss\_g50 &             rel &   top1 &     1.8 \\
         hubness &             rel &   top1 &       {\bf 2.3} \\
      hubness10k &             rel &   top1 &       2.2 \\
      hubness50k &             rel &   top1 &       2.2 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top1 &      15.4 \\
 focal\_loss\_g025 &             obj &   top1 &      14.8 \\
   focal\_loss\_g1 &             obj &   top1 &      15.2 \\
  focal\_loss\_g10 &             obj &   top1 &      15.4 \\
   focal\_loss\_g2 &             obj &   top1 &      15.0 \\
   focal\_loss\_g5 &             obj &   top1 &      15.5 \\
  focal\_loss\_g50 &             obj &   top1 &      13.7 \\
         hubness &             obj &   top1 &      15.6 \\
      hubness10k &             obj &   top1 &      {\bf 15.9} \\
      hubness50k &             obj &   top1 &      15.4 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top1 &      15.3 \\
 focal\_loss\_g025 &             sbj &   top1 &      14.6 \\
   focal\_loss\_g1 &             sbj &   top1 &      15.1 \\
  focal\_loss\_g10 &             sbj &   top1 &      15.3 \\
   focal\_loss\_g2 &             sbj &   top1 &      14.9 \\
   focal\_loss\_g5 &             sbj &   top1 &      15.3 \\
  focal\_loss\_g50 &             sbj &   top1 &      13.6 \\
         hubness &             sbj &   top1 &      15.4 \\
      hubness10k &             sbj &   top1 &      {\bf 15.7} \\
      hubness50k &             sbj &   top1 &      15.3 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top5 &       8.6 \\
 focal\_loss\_g025 &             rel &   top5 &       5.3 \\
   focal\_loss\_g1 &             rel &   top5 &       5.4 \\
  focal\_loss\_g10 &             rel &   top5 &       6.5 \\
   focal\_loss\_g2 &             rel &   top5 &       5.7 \\
   focal\_loss\_g5 &             rel &   top5 &       5.8 \\
  focal\_loss\_g50 &             rel &   top5 &       6.4 \\
         hubness &             rel &   top5 &       {\bf 8.7} \\
      hubness10k &             rel &   top5 &       8.3 \\
      hubness50k &             rel &   top5 &       8.2 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top5 &      41.2 \\
 focal\_loss\_g025 &             obj &   top5 &      40.4 \\
   focal\_loss\_g1 &             obj &   top5 &      40.8 \\
  focal\_loss\_g10 &             obj &   top5 &      40.7 \\
   focal\_loss\_g2 &             obj &   top5 &      40.7 \\
   focal\_loss\_g5 &             obj &   top5 &      40.6 \\
  focal\_loss\_g50 &             obj &   top5 &      38.9 \\
         hubness &             obj &   top5 &      {\bf 42.0} \\
      hubness10k &             obj &   top5 &      41.6 \\
      hubness50k &             obj &   top5 &      41.0 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top5 &      41.1 \\
 focal\_loss\_g025 &             sbj &   top5 &      40.3 \\
   focal\_loss\_g1 &             sbj &   top5 &      40.8 \\
  focal\_loss\_g10 &             sbj &   top5 &      40.7 \\
   focal\_loss\_g2 &             sbj &   top5 &      40.6 \\
   focal\_loss\_g5 &             sbj &   top5 &      40.6 \\
  focal\_loss\_g50 &             sbj &   top5 &      38.7 \\
         hubness &             sbj &   top5 &      {\bf 41.9} \\
      hubness10k &             sbj &   top5 &      41.4 \\
      hubness50k &             sbj &   top5 &      41.0 \\
\bottomrule
\end{tabular}


==> tables/fine-grained/gvqa_per_class_mean_analysis_2decimals.tex <==
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top1 &      2.28 \\
 focal\_loss\_g025 &             rel &   top1 &      1.79 \\
   focal\_loss\_g1 &             rel &   top1 &      1.79 \\
  focal\_loss\_g10 &             rel &   top1 &      1.96 \\
   focal\_loss\_g2 &             rel &   top1 &      1.76 \\
   focal\_loss\_g5 &             rel &   top1 &      1.87 \\
  focal\_loss\_g50 &             rel &   top1 &      1.77 \\
         hubness &             rel &   top1 &      {\bf 2.29} \\
      hubness10k &             rel &   top1 &      2.18 \\
      hubness50k &             rel &   top1 &      2.24 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top1 &     15.43 \\
 focal\_loss\_g025 &             obj &   top1 &     14.76 \\
   focal\_loss\_g1 &             obj &   top1 &     15.19 \\
  focal\_loss\_g10 &             obj &   top1 &     15.41 \\
   focal\_loss\_g2 &             obj &   top1 &     15.01 \\
   focal\_loss\_g5 &             obj &   top1 &     15.48 \\
  focal\_loss\_g50 &             obj &   top1 &     13.69 \\
         hubness &             obj &   top1 &     15.60 \\
      hubness10k &             obj &   top1 &     {\bf 15.88} \\
      hubness50k &             obj &   top1 &     15.41 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top1 &     15.30 \\
 focal\_loss\_g025 &             sbj &   top1 &     14.61 \\
   focal\_loss\_g1 &             sbj &   top1 &     15.05 \\
  focal\_loss\_g10 &             sbj &   top1 &     15.26 \\
   focal\_loss\_g2 &             sbj &   top1 &     14.89 \\
   focal\_loss\_g5 &             sbj &   top1 &     15.34 \\
  focal\_loss\_g50 &             sbj &   top1 &     13.56 \\
         hubness &             sbj &   top1 &     15.44 \\
      hubness10k &             sbj &   top1 &     {\bf 15.72} \\
      hubness50k &             sbj &   top1 &     15.32 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top5 &      8.61 \\
 focal\_loss\_g025 &             rel &   top5 &      5.28 \\
   focal\_loss\_g1 &             rel &   top5 &      5.38 \\
  focal\_loss\_g10 &             rel &   top5 &      6.54 \\
   focal\_loss\_g2 &             rel &   top5 &      5.68 \\
   focal\_loss\_g5 &             rel &   top5 &      5.81 \\
  focal\_loss\_g50 &             rel &   top5 &      6.40 \\
         hubness &             rel &   top5 &      {\bf 8.69} \\
      hubness10k &             rel &   top5 &      8.30 \\
      hubness50k &             rel &   top5 &      8.25 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top5 &     41.21 \\
 focal\_loss\_g025 &             obj &   top5 &     40.40 \\
   focal\_loss\_g1 &             obj &   top5 &     40.84 \\
  focal\_loss\_g10 &             obj &   top5 &     40.72 \\
   focal\_loss\_g2 &             obj &   top5 &     40.72 \\
   focal\_loss\_g5 &             obj &   top5 &     40.62 \\
  focal\_loss\_g50 &             obj &   top5 &     38.85 \\
         hubness &             obj &   top5 &     {\bf 42.00} \\
      hubness10k &             obj &   top5 &     41.61 \\
      hubness50k &             obj &   top5 &     41.00 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top5 &     41.07 \\
 focal\_loss\_g025 &             sbj &   top5 &     40.28 \\
   focal\_loss\_g1 &             sbj &   top5 &     40.77 \\
  focal\_loss\_g10 &             sbj &   top5 &     40.66 \\
   focal\_loss\_g2 &             sbj &   top5 &     40.63 \\
   focal\_loss\_g5 &             sbj &   top5 &     40.65 \\
  focal\_loss\_g50 &             sbj &   top5 &     38.67 \\
         hubness &             sbj &   top5 &     {\bf 41.95} \\
      hubness10k &             sbj &   top5 &     41.44 \\
      hubness50k &             sbj &   top5 &     40.97 \\
\bottomrule
\end{tabular}






==> tables/fine-grained/gvqa_simple_mean_analysis.tex <==
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top1 &      48.8 \\
 focal\_loss\_g025 &             rel &   top1 &      48.6 \\
   focal\_loss\_g1 &             rel &   top1 &      48.7 \\
  focal\_loss\_g10 &             rel &   top1 &      48.5 \\
   focal\_loss\_g2 &             rel &   top1 &      48.7 \\
   focal\_loss\_g5 &             rel &   top1 &      48.8 \\
  focal\_loss\_g50 &             rel &   top1 &      48.3 \\
         hubness &             rel &   top1 &      {\bf 49.0} \\
      hubness10k &             rel &   top1 &      48.9 \\
      hubness50k &             rel &   top1 &      48.9 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top1 &      52.5 \\
 focal\_loss\_g025 &             obj &   top1 &      {\bf 53.1} \\
   focal\_loss\_g1 &             obj &   top1 &      52.8 \\
  focal\_loss\_g10 &             obj &   top1 &      50.5 \\
   focal\_loss\_g2 &             obj &   top1 &      52.5 \\
   focal\_loss\_g5 &             obj &   top1 &      51.7 \\
  focal\_loss\_g50 &             obj &   top1 &      50.0 \\
         hubness &             obj &   top1 &      52.1 \\
      hubness10k &             obj &   top1 &      52.4 \\
      hubness50k &             obj &   top1 &      52.3 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top1 &      52.0 \\
 focal\_loss\_g025 &             sbj &   top1 &      {\bf 52.6} \\
   focal\_loss\_g1 &             sbj &   top1 &      52.4 \\
  focal\_loss\_g10 &             sbj &   top1 &      50.1 \\
   focal\_loss\_g2 &             sbj &   top1 &      52.1 \\
   focal\_loss\_g5 &             sbj &   top1 &      51.3 \\
  focal\_loss\_g50 &             sbj &   top1 &      49.6 \\
         hubness &             sbj &   top1 &      51.6 \\
      hubness10k &             sbj &   top1 &      51.9 \\
      hubness50k &             sbj &   top1 &      51.9 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top5 &      {\bf 97.3} \\
 focal\_loss\_g025 &             rel &   top5 &      96.9 \\
   focal\_loss\_g1 &             rel &   top5 &      96.9 \\
  focal\_loss\_g10 &             rel &   top5 &      96.8 \\
   focal\_loss\_g2 &             rel &   top5 &      96.9 \\
   focal\_loss\_g5 &             rel &   top5 &      96.9 \\
  focal\_loss\_g50 &             rel &   top5 &      96.3 \\
         hubness &             rel &   top5 &      {\bf 97.3} \\
      hubness10k &             rel &   top5 &      {\bf 97.3} \\
      hubness50k &             rel &   top5 &      {\bf 97.3} \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top5 &      81.5 \\
 focal\_loss\_g025 &             obj &   top5 &      {\bf 81.9} \\
   focal\_loss\_g1 &             obj &   top5 &      {\bf 81.9} \\
  focal\_loss\_g10 &             obj &   top5 &      81.2 \\
   focal\_loss\_g2 &             obj &   top5 &      {\bf 81.9} \\
   focal\_loss\_g5 &             obj &   top5 &      81.8 \\
  focal\_loss\_g50 &             obj &   top5 &      80.4 \\
         hubness &             obj &   top5 &      81.5 \\
      hubness10k &             obj &   top5 &      81.4 \\
      hubness50k &             obj &   top5 &      81.5 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top5 &      81.3 \\
 focal\_loss\_g025 &             sbj &   top5 &      81.7 \\
   focal\_loss\_g1 &             sbj &   top5 &      {\bf 81.8} \\
  focal\_loss\_g10 &             sbj &   top5 &      81.0 \\
   focal\_loss\_g2 &             sbj &   top5 &      81.7 \\
   focal\_loss\_g5 &             sbj &   top5 &      81.6 \\
  focal\_loss\_g50 &             sbj &   top5 &      80.1 \\
         hubness &             sbj &   top5 &      81.2 \\
      hubness10k &             sbj &   top5 &      81.2 \\
      hubness50k &             sbj &   top5 &      81.3 \\
\bottomrule
\end{tabular}


==> tables/fine-grained/gvqa_simple_mean_analysis_2decimals.tex <==
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top1 &     48.85 \\
 focal\_loss\_g025 &             rel &   top1 &     48.62 \\
   focal\_loss\_g1 &             rel &   top1 &     48.70 \\
  focal\_loss\_g10 &             rel &   top1 &     48.52 \\
   focal\_loss\_g2 &             rel &   top1 &     48.68 \\
   focal\_loss\_g5 &             rel &   top1 &     48.76 \\
  focal\_loss\_g50 &             rel &   top1 &     48.27 \\
         hubness &             rel &   top1 &     {\bf 49.00} \\
      hubness10k &             rel &   top1 &     48.94 \\
      hubness50k &             rel &   top1 &     48.93 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top1 &     52.45 \\
 focal\_loss\_g025 &             obj &   top1 &     {\bf 53.05} \\
   focal\_loss\_g1 &             obj &   top1 &     52.77 \\
  focal\_loss\_g10 &             obj &   top1 &     50.54 \\
   focal\_loss\_g2 &             obj &   top1 &     52.45 \\
   focal\_loss\_g5 &             obj &   top1 &     51.74 \\
  focal\_loss\_g50 &             obj &   top1 &     49.96 \\
         hubness &             obj &   top1 &     52.09 \\
      hubness10k &             obj &   top1 &     52.39 \\
      hubness50k &             obj &   top1 &     52.33 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top1 &     52.00 \\
 focal\_loss\_g025 &             sbj &   top1 &     {\bf 52.62} \\
   focal\_loss\_g1 &             sbj &   top1 &     52.35 \\
  focal\_loss\_g10 &             sbj &   top1 &     50.13 \\
   focal\_loss\_g2 &             sbj &   top1 &     52.06 \\
   focal\_loss\_g5 &             sbj &   top1 &     51.34 \\
  focal\_loss\_g50 &             sbj &   top1 &     49.56 \\
         hubness &             sbj &   top1 &     51.65 \\
      hubness10k &             sbj &   top1 &     51.95 \\
      hubness50k &             sbj &   top1 &     51.95 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             rel &   top5 &     {\bf 97.32} \\
 focal\_loss\_g025 &             rel &   top5 &     96.89 \\
   focal\_loss\_g1 &             rel &   top5 &     96.90 \\
  focal\_loss\_g10 &             rel &   top5 &     96.83 \\
   focal\_loss\_g2 &             rel &   top5 &     96.92 \\
   focal\_loss\_g5 &             rel &   top5 &     96.92 \\
  focal\_loss\_g50 &             rel &   top5 &     96.33 \\
         hubness &             rel &   top5 &     97.30 \\
      hubness10k &             rel &   top5 &     97.27 \\
      hubness50k &             rel &   top5 &     97.30 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             obj &   top5 &     81.49 \\
 focal\_loss\_g025 &             obj &   top5 &     81.89 \\
   focal\_loss\_g1 &             obj &   top5 &     {\bf 81.92} \\
  focal\_loss\_g10 &             obj &   top5 &     81.19 \\
   focal\_loss\_g2 &             obj &   top5 &     81.91 \\
   focal\_loss\_g5 &             obj &   top5 &     81.80 \\
  focal\_loss\_g50 &             obj &   top5 &     80.35 \\
         hubness &             obj &   top5 &     81.46 \\
      hubness10k &             obj &   top5 &     81.42 \\
      hubness50k &             obj &   top5 &     81.54 \\
\bottomrule
\end{tabular}
\begin{tabular}{lllr}
\toprule
          method & prediction-type & metric &  accuracy \\
\midrule
        baseline &             sbj &   top5 &     81.26 \\
 focal\_loss\_g025 &             sbj &   top5 &     81.66 \\
   focal\_loss\_g1 &             sbj &   top5 &     {\bf 81.75} \\
  focal\_loss\_g10 &             sbj &   top5 &     80.99 \\
   focal\_loss\_g2 &             sbj &   top5 &     81.72 \\
   focal\_loss\_g5 &             sbj &   top5 &     81.60 \\
  focal\_loss\_g50 &             sbj &   top5 &     80.12 \\
         hubness &             sbj &   top5 &     81.24 \\
      hubness10k &             sbj &   top5 &     81.21 \\
      hubness50k &             sbj &   top5 &     81.34 \\
\bottomrule
\end{tabular}



==> tables/gqa_many_median_few_pc.tex <==
\begin{table*}[t!]
\centering
\caption{\label{tab:many_medium_few_gqa_pc} Performance on GQA}
\scalebox{0.8}
{
\begin{tabular}{l|cccc|cccc}
\toprule
{}              & \multicolumn{4}{c}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
\midrule
Model &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
\cite{zhang2019large}            &       64.2 &         29.6 &       1.0 &       8.5 &       43.0 &          5.1 &       0.1 &       3.0 \\
\cite{zhang2019large} + ViLHub 10k                     &       64.7 &         32.4 &       1.5 &       9.3 &       46.2 &          7.2 &       0.2 &       3.6 \\
\cite{zhang2019large} + ViLHub 50k                     &       64.7 &         35.8 &       2.6 &      10.7 &       46.3 &          5.5 &       0.1 &       3.3 \\
\cite{zhang2019large} + ViLHub 100k                    &       64.7 &         36.6 &       3.1 &      11.2 &       46.4 &          4.7 &       0.1 &       3.2 \\
\midrule
FL~\cite{lin2017focal}                    &       64.1 &         31.8 &       1.4 &       9.1 &       40.3 &          5.4 &       0.0 &       2.9 \\
FL + ViLHub20k                            &       64.7 &         36.2 &       2.8 &      10.9 &       46.0 &          4.4 &       0.1 &       3.1 \\
\midrule
WCE                                       &       45.2 &         34.2 &       8.0 &      13.8 &       38.9 &         29.5 &       8.2 &      13.0 \\
WCE + ViLHub                              &       43.1 &         37.2 &       9.8 &      15.6 &       39.1 &         32.8 &       8.4 &      13.6 \\
\midrule
FC                                        &       64.5 &         19.1 &       0.0 &       6.1 &       29.8 &          0.0 &       0.0 &       1.5 \\
FC + ViLHub100k                           &       65.7 &         24.1 &       0.1 &       7.0 &       36.2 &          0.0 &       0.0 &       1.9 \\
\midrule
DCPL$_\tau$~\cite{Kang2020Decoupling}     &       63.8 &         19.3 &       0.0 &       6.1 &       29.1 &          0.0 &       0.0 &       1.5 \\
DCPL$_m$                                  &       60.1 &         28.2 &       1.2 &       8.2 &       45.9 &         15.3 &       0.1 &       4.7 \\
DCPL$_m$ + ViLHub100k                     &       59.6 &         32.5 &       1.9 &       9.4 &       45.4 &         17.9 &       0.2 &       5.2 \\
\midrule
OLTR~\cite{liu2019large}           &       64.1 &         29.9 &       1.0 &       8.5 &       42.7 &          5.4 &       0.1 &       3.1 \\
EQL~\cite{9157168}            &       64.7 &         36.4 &       3.1 &      11.2 &       46.6 &          4.7 &       0.1 &       3.2 \\
\cite{zhang2019large} + Bert  &       64.1 &         29.9 &       1.0 &       8.5 &       42.7 &          5.4 &       0.1 &       3.1 \\

\bottomrule         
\end{tabular}
}
\end{table*}


==> tables/gqa_many_median_few_pc_syn.tex <==
% \begin{table*}[t!]
% \centering
% \caption{\label{tab:gqa_many_median_few_pc_syn} Performance on GQA based on Synsets}
% \scalebox{0.8}
% {
% \begin{tabular}{l|cccc|cccc}
% \toprule
% {}              & \multicolumn{4}{c}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
% \midrule
% Model &  many &  medium &  few &  all &  many &  medium &  few &  all \\
% \midrule
% \cite{zhang2019large}                       &        27.7 &           5.5 &        3.0 &       14.5 &       36.4 &         11.2 &       6.4 &      11.0 \\
% \cite{zhang2019large}  + ViLHub 10k         &        29.7 &           6.2 &        4.0 &       15.8 &       39.1 &         10.6 &       7.0 &      11.6 \\
% % \cite{zhang2019large}  + ViLHub 50k         &        68.9 &          43.1 &        9.2 &       17.3 &       63.2 &         15.4 &       7.0 &      11.2 \\
% % \cite{zhang2019large}  + ViLHub 100k        &        68.9 &          43.8 &        9.9 &       18.0 &       63.2 &         14.6 &       7.1 &      11.1 \\
% \Delta                                      &         2.0 &           0.7 &        1.0 &        1.3 &        2.7 &         -0.6 &       0.6 &       0.6 \\                          
% \midrule
% FL~\cite{lin2017focal}                      &        29.3 &           6.0 &        3.1 &       15.3 &       36.0 &         11.5 &       7.3 &      11.6 \\
% FL + ViLHub20k                              &        33.3 &           7.0 &        3.8 &       17.5 &       36.7 &          9.5 &       7.4 &      11.4 \\
% \Delta                                      &         4.0 &           1.0 &        0.7 &        2.2 &        0.7 &         -2.0 &       0.1 &      -0.2 \\
% \midrule
% WCE                                         &        34.8 &          12.2 &        4.5 &       20.2 &       44.5 &         29.7 &      14.0 &      20.5 \\
% WCE + ViLHub                                &        37.1 &          14.0 &        6.0 &       22.1 &       45.9 &         34.5 &      13.4 &      21.2 \\
% \Delta                                      &         2.3 &           1.8 &        1.5 &        1.9 &        1.4 &          4.8 &      -0.6 &       0.7 \\ 
% \midrule
% FC                                          &        21.5 &           4.9 &        2.6 &       11.5 &       26.2 &          8.5 &       5.4 &       8.5 \\
% FC + ViLHub100k                             &        24.1 &           5.1 &        2.6 &       12.7 &       27.6 &          7.9 &       5.2 &       8.4 \\
% \Delta                                      &         2.6 &           0.2 &        0.0 &        1.2 &        1.4 &         -0.6 &      -0.2 &      -0.1 \\
% \midrule
% % DCPL$_\tau$~\cite{Kang2020Decoupling}       &        68.1 &          26.0 &        5.1 &       11.4 &       49.5 &          9.0 &       5.4 &       8.2 \\
% DCPL$_m$~\cite{Kang2020Decoupling}          &        26.4 &           5.3 &        2.2 &       13.7 &       42.6 &         14.1 &       7.1 &      12.7 \\
% DCPL$_m$ + ViLHub100k                       &        29.4 &           5.8 &        2.5 &       15.2 &       43.5 &         15.6 &       6.2 &      12.5 \\
% \Delta                                      &         3.0 &           0.5 &        0.3 &        1.5 &        0.9 &          1.5 &      -0.9 &      -0.2 \\
% \midrule
% OLTR~\cite{liu2019large}                    &        27.9 &           5.8 &        3.0 &       14.6 &       36.6 &         11.4 &       6.1 &      10.8 \\
% EQL~\cite{9157168}                          &        33.8 &           7.2 &        4.6 &       18.0 &       37.5 &          9.5 &       8.2 &      12.1 \\

% \bottomrule         
% \end{tabular}
% }
% \end{table*}


\begin{table}[t!]
\parbox{.5\linewidth}{
\centering
\caption{\label{tab:gqa_many_median_few_pc_syn} Performance on GQA based on Synsets}
\scalebox{0.5}
{
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
{}              & \multicolumn{4}{c}{sbj/obj} & \multicolumn{4}{|c}{rel}\\
\midrule
Model &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
\cite{zhang2019large}                       &        68.3 &          37.0 &        6.9 &       14.5 &       62.6 &         15.5 &       6.8 &      11.0 \\
\cite{zhang2019large}  + ViLHub 10k         &        68.8 &          39.7 &        8.0 &       15.8 &       63.6 &         17.3 &       7.2 &      11.6 \\
% \cite{zhang2019large}  + ViLHub 50k         &        68.9 &          43.1 &        9.2 &       17.3 &       63.2 &         15.4 &       7.0 &      11.2 \\
% \cite{zhang2019large}  + ViLHub 100k        &        68.9 &          43.8 &        9.9 &       18.0 &       63.2 &         14.6 &       7.1 &      11.1 \\
\Delta                                      &         \bf+0.5 &           \bf+2.7 &        \bf+1.1 &        \bf+1.3 &        \bf+1.0 &          \bf+1.8 &       \bf+0.4 &       \bf+0.6 \\                          
\midrule
FL~\cite{lin2017focal}                      &        68.2 &          39.2 &        7.5 &       15.3 &       60.4 &         15.7 &       7.7 &      11.6 \\
FL + ViLHub20k                              &        69.0 &          43.4 &        9.5 &       17.5 &       63.1 &         14.2 &       7.5 &      11.4 \\
\Delta                                      &         \bf+0.8 &           \bf+4.2 &        \bf+2.0 &        \bf+2.2 &        \bf+2.7 &         \bf-1.5 &      \bf-0.2 &      \bf-0.2 \\
\midrule
WCE                                         &        53.4 &          42.0 &       14.0 &       20.2 &       53.4 &         35.1 &      15.7 &      20.5 \\
WCE + ViLHub                                &        52.0 &          44.6 &       16.0 &       22.1 &       53.1 &         39.0 &      15.8 &      21.2 \\
\Delta                                      &        \bf-1.4 &           \bf+2.6 &        \bf+2.0 &        \bf+1.9 &       \bf-0.3 &          \bf+3.9 &       \bf+0.1 &       \bf+0.7 \\ 
\midrule
FC                                          &        68.7 &          26.0 &        5.2 &       11.5 &       49.9 &          9.0 &       5.8 &       8.5 \\
FC + ViLHub100k                              &        69.7 &          31.4 &        5.6 &       12.7 &       54.1 &          8.7 &       5.4 &       8.4 \\
\Delta                                      &         \bf+1.0 &           \bf+5.4 &        \bf+0.4 &        \bf+1.2 &        \bf+4.2 &         \bf-0.3 &      \bf-0.4 &      \bf-0.1 \\
\midrule
% DCPL$_\tau$~\cite{Kang2020Decoupling}       &        68.1 &          26.0 &        5.1 &       11.4 &       49.5 &          9.0 &       5.4 &       8.2 \\
DCPL$_m$~\cite{Kang2020Decoupling}          &        64.0 &          35.3 &        6.4 &       13.7 &       61.4 &         23.6 &       7.6 &      12.7 \\
DCPL$_m$ + ViLHub100k                       &        63.5 &          39.8 &        7.5 &       15.2 &       58.6 &         26.1 &       7.0 &      12.5 \\
\Delta                                      &        \bf-0.5 &           \bf+4.5 &        \bf+1.1 &        \bf+1.5 &       \bf-2.8 &          \bf+2.5 &      \bf-0.6 &      \bf-0.2 \\
\midrule
OLTR~\cite{liu2019large}                    &        68.2 &          37.2 &        7.0 &       14.6 &       62.3 &         15.8 &       6.6 &      10.8 \\
EQL~\cite{9157168}                          &        68.9 &          43.7 &       10.0 &       18.0 &       63.5 &         15.0 &       8.2 &      12.1 \\

\bottomrule         
\end{tabular}
}
}
\end{table}


==> tables/gqa_many_median_few_syn.tex <==
\begin{table}[ht!]
\centering
% \vspace{-10mm}

\caption{\label{tab:many_medium_few_syn} Performance on GQA with Synset Matching}
\scalebox{0.8}
{
\begin{tabular}{l|cccc|cccc}
\toprule
{}              & \multicolumn{4}{c}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
\midrule
Model &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
Baseline~\cite{zhang2019large}                         &    \bf73.0 &      42.4 &   11.6 &   56.2 &    \bf96.5 &      15.5 &    \bf8.1 &   \bf94.7 \\
Baseline + ViLHub 10k           &    72.9 &      45.0 &   13.2 &   57.1 &    94.4 &      \bf18.6 &    \bf8.1 &   92.7 \\
Baseline + ViLHub 50k           &    72.6 &      47.6 &   16.1 &   58.0 &    93.4 &      17.3 &    8.0 &   91.7 \\
Baseline + ViLHub 100k          &    72.6 &      \bf48.2 &   \bf17.3 &   \bf58.4 &    92.8 &      16.3 &    7.9 &   91.1 \\
\midrule
FL~\cite{lin2017focal}                              &    71.9 &      44.8 &   13.2 &   56.5 &    \bf96.4 &      15.1 &    \bf8.2 &   \bf94.6 \\
FL + ViLHub20k                  &    \bf72.5 &      \bf48.0 &   \bf16.7 &   \bf58.2 &    93.4 &      \bf15.9 &    \bf8.2 &   91.7 \\
\midrule

WCE                             &    \bf47.6 &      44.3 &   22.9 &   \bf43.4 &    \bf72.6 &      34.0 &   22.1 &   \bf71.7 \\
WCE + ViLHub                    &    43.9 &      \bf46.9 &   \bf25.5 &   42.3 &    69.1 &      \bf37.0 &   \bf23.8 &   68.3 \\
\midrule

FC                              &    \bf74.1 &      32.7 &    7.1 &   \bf53.5 &    96.1 &       9.0 &    6.4 &   \bf94.3 \\
DCPL$_\tau$~\cite{Kang2020Decoupling}                     &    73.9 &      32.7 &    7.0 &   53.4 &    \bf96.2 &       9.1 &    6.2 &   \bf94.3 \\
DCPL$_m$~\cite{Kang2020Decoupling}                        &    65.0 &      40.1 &   11.4 &   50.9 &    89.3 &      24.9 &    9.1 &   87.8 \\
DCPL$_m$ + ViLHub100k           &    62.3 &      \bf44.3 &   \bf13.6 &   50.8 &    78.7 &      \bf27.8 &    \bf9.2 &   77.5 \\
\end{tabular}
}
\end{table}


==> tables/gqa_triplet.tex <==
\begin{table}
\centering
\caption{\label{tab:gvqa_triplets}Triplet Scores on GQA using Synsets}
\scalebox{0.7}
{
\begin{tabular}{lrrrr}
\toprule
Model &  many &  median &   few &   all \\
\midrule
\cite{zhang2019large}                   &  42.8 &    25.8 &   9.0 &  13.2 \\
\cite{zhang2019large} + ViLHub 10k      &  43.5 &    27.5 &   9.7 &  14.1 \\
\Delta                                  &   \bf+0.7 &     \bf+1.7 &   \bf+0.7 &   \bf+0.9 \\
\midrule
FL~\cite{lin2017focal}                  &  43.2 &    27.5 &   9.7 &  14.1 \\
FL + ViLHub                             &  44.4 &    29.8 &  11.5 &  15.9 \\
\Delta                                  &   \bf+1.2 &     \bf+2.3 &   \bf+1.8 &   \bf+1.8 \\
\midrule
WCE                                     &  19.4 &    14.8 &   7.6 &   9.2 \\
WCE + ViLHub                            &  18.0 &    14.8 &   7.9 &   9.4 \\
\Delta                                  &  \bf-1.4 &     \bf0.0 &   \bf+0.3 &   \bf+0.2 \\
\midrule
FC                                      &  39.2 &    20.4 &   6.3 &  10.0 \\
FC + ViLHub                             &  41.8 &    23.4 &   7.3 &  11.5 \\
\Delta                                  &   \bf+2.6 &     \bf+3.0 &   \bf+1.0 &   \bf+1.5 \\
\midrule
DCPL~\cite{Kang2020Decoupling}          &  33.7 &    20.2 &   7.3 &  10.6 \\
DCPL + ViLHub                           &  29.3 &    19.6 &   7.8 &  10.6 \\
\Delta                                  &  \bf-4.4 &    \bf-0.6 &   \bf+0.5 &   \bf0.0 \\
\midrule
OLTR                                    &  42.6 &    26.0 &   9.1 &  13.3 \\
EQL                                     &  44.4 &    30.0 &  11.7 &  16.0 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/gqa_triplet_scores.tex <==
\begin{table}
\centering
\caption{\label{tab:gvqa_triplets}Accuracy on Relation Triplets on GQA using Synsets}
\scalebox{0.7}{
\begin{tabular}{lrrrr}
\toprule
Model &  many &  medium &   few &   all \\
\midrule
LSVRU~\cite{zhang2019large}            &  42.8 &    25.8 &   9.0 &  13.2 \\
LSVRU + ViLHub             &  44.3 &    30.0 &  11.7 &  16.0 \\
$\Delta$            &   \bf+1.5 &     \bf+4.2 &   \bf+2.7 &   \bf+2.8 \\
\midrule
FL~\cite{lin2017focal}            &  43.2 &    27.5 &   9.7 &  14.1 \\
FL + ViLHub    &  44.4 &    29.8 &  11.5 &  15.9 \\
$\Delta$            &   \bf+1.2 &     \bf+2.3 &   \bf+1.8 &   \bf+1.8 \\
\midrule
WCE               &  19.4 &    14.8 &   7.6 &   9.2 \\
WCE + ViLHub       &  18.0 &    14.8 &   7.9 &   9.4 \\
$\Delta$            &  \bf-1.4 &     \bf0.0 &   \bf+0.3 &   \bf+0.2 \\
\midrule
FC                  &  39.2 &    20.4 &   6.3 &  10.0 \\
FC + ViLHub         &  41.8 &    23.4 &   7.3 &  11.5 \\
$\Delta$            &   \bf+2.6 &     \bf+3.0 &   \bf+1.0 &   \bf+1.5 \\
\midrule
DCPL                &  33.7 &    20.2 &   7.3 &  10.6 \\
DCPL + ViLHub       &  29.3 &    19.6 &   7.8 &  10.6 \\
$\Delta$            &  \bf-4.4 &    \bf-0.6 &   \bf+0.5 &   \bf0.0 \\
\midrule
OLTR                &  42.6 &    26.0 &   9.1 &  13.3 \\
EQL                 &  44.4 &    30.0 &  11.7 &  16.0 \\
% \midrule
% LSVRU               &  42.8 &    25.8 &   9.0 &  13.2 \\
% LSVRU + RelMix     &  42.6 &    26.3 &   9.7 &  13.9 \\
% $\Delta$            &  \bf-0.2 &     \bf+0.5 &   \bf+0.7 &   \bf+0.6 \\
% % 100k                 &  44.4 &    29.9 &  11.6 &  16.0 \\
% LSVRU + RelMix + ViLHub     &  44.3 &    30.0 &  11.7 &  16.1 \\
% $\Delta$            &   \bf+1.5 &     \bf+4.2 &   \bf+2.7 &   \bf+0.1 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/gqa_vg8k_relmix_results.tex <==
\begin{table}[th!]
\parbox{.9\linewidth}{
\centering
\caption{\label{tab:relmix_results} Average Per-class Accuracy using Relmix on GQA and VG8K}
\scalebox{0.5}
{
\begin{tabular}{|l|l|cccc|cccc|}
\toprule
{} & {}            & \multicolumn{4}{c}{sbj/obj} & \multicolumn{4}{|c|}{rel}\\
\midrule
Dataset & Model &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
                    & LSVRU                  &        68.2 &          37.2 &        7.0 &       14.6 &       62.2 &         15.7 &       6.5 &      10.8 \\
                    & LSVRU+Relmix           &        68.2 &          37.7 &        9.3 &       16.5 &       62.3 &         16.0 &       6.6 &      10.9 \\
GQA-LT              & $\Delta$               &         \bf+0.0 &           \bf+0.5 &        \bf+2.3 &        \bf+1.9 &        \bf+0.1 &          \bf+0.3 &       \bf+0.1 &       \bf+0.1 \\
                    & LSVRU+Relmix+ViLHub    &        68.8 &          42.1 &       10.1 &       18.1 &       63.4 &         14.9 &       8.0 &      11.9 \\
                    & $\Delta$               &         \bf+0.6 &           \bf+4.9 &        \bf+3.1 &        \bf+3.5  &        \bf+1.2 &         \bf-0.8 &       \bf+1.5 &       \bf+1.1 \\
\bottomrule
                    & LSVRU                 &        57.3 &          11.1 &        8.5 &       11.4 &       22.2 &         15.5 &      12.6 &      13.5 \\
                    & LSVRU+Relmix          &        56.9 &          12.4 &       10.3 &       13.0 &       22.7 &         15.6 &      12.6 &      13.6 \\
VG8K-LT             & $\Delta$              &        \bf-0.4 &           \bf+1.3 &        \bf+1.8 &        \bf+1.6 &        \bf+0.5 &          \bf+0.1 &       0.0 &       \bf+0.1 \\
                    & LSVRU+Relmix+ViLHub   &        59.5 &          15.1 &       10.4 &       13.6 &       24.5 &         16.5 &      14.4 &      15.4 \\
                    & $\Delta$              &         \bf+2.2 &           \bf+4.0 &        \bf+1.9 &        \bf+2.2 &        \bf+2.3 &          \bf+1.0 &       \bf+1.8 &       \bf+1.9 \\
\bottomrule
\end{tabular}
}
}
\end{table}

% \midrule
% LSVRU                     &        68.3 &          37.0 &        6.9 &       14.5 &       62.6 &         15.5 &       6.8 &      11.0 \\
% LSVRU + RelMix            &        68.2 &          37.7 &        9.3 &       16.5 &       62.3 &         16.0 &       6.6 &      10.9 \\
% $\Delta$                  &        \bf0.0 &           \bf+0.5 &        \bf+2.3 &        \bf+2.3 &        \bf+0.1 &          \bf+0.3 &       \bf+0.1 &       \bf+0.1 \\
% LSVRU + RelMix + ViLHub   &        68.8 &          43.9 &       10.1 &       18.1 &       63.4 &         14.9 &       8.0 &      11.9 \\
% $\Delta$                  &        \bf-0.1 &           \bf+0.7 &        \bf+2.4 &        \bf+1.9 &       \bf-0.3 &          \bf+0.5 &      \bf-0.2 &       \bf+0.1 \\

% \midrule
% LSVRU                     &        57.3 &          11.1 &        8.5 &       11.4 &       22.2 &         15.5 &      12.6 &      13.5 \\
% RelMix                    &       56.9 &          12.4 &       10.3 &       13.0 &       22.7 &         15.6 &      12.6 &      13.6 \\
% $\Delta$                  &        \bf-0.4 &           \bf+1.3 &        \bf+1.8 &        \bf+1.6 &        \bf+0.5 &          \bf+0.1 &       0.0 &       \bf+0.1 \\
% \midrule
% LSVRU                     &       57.3 &          11.1 &        8.5 &       11.4 &       22.2 &         15.5 &      12.6 &      13.5 \\
% RelMix + VilHub           &       60.3 &          15.1 &       10.4 &       13.6 &       27.9 &         16.5 &      14.4 &      15.4 \\
% $\Delta$                  &       \bf+3.0 &           \bf+4.0 &        \bf+1.9 &        \bf+1.0 &        \bf+5.7 &          \bf+1.0 &       \bf+1.8 &       \bf+0.1 \\


==> tables/gqa_wordsim.tex <==
\begin{table}[ht!]
\centering
\caption{\label{tab:per_class_wordsim} Per-class word similarity on subjects/objects in GQA}
\scalebox{0.8}
{
\begin{tabular}{l|ccccc}
\toprule
% {}              & \multicolumn{5}{c|}{sbj/obj}  \\
% \midrule
Models &  lch &  wup &  lin &  path &  w2v  \\
\midrule
Baseline~\cite{zhang2019large}                        &     51.2 &     59.4 &     36.8 &      27.5 &     45.2  \\
Baseline + ViLHub 10k           &     52.0 &     60.1 &     37.8 &      28.6 &     45.8  \\
Baseline + ViLHub 50k           &     53.1 &     61.0 &     39.0 &      30.1 &     46.7  \\
Baseline + ViLHub 100k          &     \bf53.4 &     \bf61.3 &     \bf39.5 &      \bf30.6 &     \bf47.1  \\
\midrule
FL~\cite{lin2017focal}                              &     51.8 &     60.0 &     37.5 &      28.3 &     45.7  \\
FL + ViLHub20k                  &     \bf53.2 &     \bf61.1 &     \bf39.1 &      \bf30.3 &     \bf47.0  \\
\midrule
WCE                             &     53.5 &     61.1 &     39.4 &      31.8 &     47.8  \\
WCE + ViLHub                    &     \bf54.8 &     \bf62.1 &     \bf41.0 &      \bf33.5 &     \bf49.2  \\
\midrule
FC                              &     48.9 &     57.1 &     33.8 &      24.5 &     43.3  \\
DCPL$_\tau$~\cite{Kang2020Decoupling}                     &     49.0 &     57.3 &     33.9 &      24.5 &     43.2  \\
DCPL$_m$~\cite{Kang2020Decoupling}                        &     49.1 &     57.4 &     34.1 &      25.8 &     43.0  \\
DCPL$_m$ + ViLHub100k           &     \bf50.4 &     \bf58.4 &     \bf35.5 &      \bf27.3 &     \bf44.7  \\
\bottomrule
\end{tabular}
}
\end{table}


% &     52.1
% &     51.8
% &     51.4
% &     51.3
% &     51.7
% &     51.4
% &     47.4
% &     46.7
% &     51.6
% &     51.6
% &     50.5
% &     48.7

==> tables/gvqa_combined_metrics.tex <==
\begin{table*}[ht!]
\centering
% \vspace{-3mm}
\caption{\label{tab:combined_performance} Performance on GQA}
\scalebox{0.8}
{
\begin{tabular}{l|cc|cc|c|cc|cc}
\toprule
 {}                             &      \multicolumn{5}{|c|}{Overall}                        & \multicolumn{4}{|c}{Per-class} \\
\midrule
 {}                             & \multicolumn{2}{|c|}{sbj/obj} & \multicolumn{2}{|c|}{rel} & triplet  & \multicolumn{2}{|c|}{sbj/obj} & \multicolumn{2}{|c}{rel}  \\
\midrule
Model                                   &   acc     &   mr      & acc   &  mr   & acc                               & acc & mr  & acc &  mr       \\ 
\midrule
Baseline~\cite{zhang2019large}          &    51.9 &   14.6 &    \bf49.7 &    \bf1.0 &    14.7 &     8.5 &  165.8 &     3.0 &   \bf72.2       \\  
Baseline + ViLHub 10k                   &     52.8 &    14.0 &     48.9 &     3.0 &     14.9 &      9.3 &   156.1 &      \bf3.6 &    76.0   \\
Baseline + ViLHub 50k                   &     53.6 &    13.0 &     48.1 &     5.3 &     15.2 &     10.7 &   136.2 &      3.3 &    77.3 \\
Baseline + ViLHub 100k                  &    \bf53.9 &   \bf12.9 &    47.9 &    6.6 &    \bf15.3 &    \bf11.3 &  \bf125.3 &     3.2 &   77.3     \\
\midrule
FL~\cite{lin2017focal}                  &    51.8 &    15.0 &     \bf49.4 &     \bf1.1 &     14.5 &      9.3 &   169.6 &      2.7 &    \bf73.5      \\
FL + ViLHub20k                          &     \bf53.8 &    \bf13.6 &     48.1 &     5.1 &     \bf15.3 &     \bf11.0 &   \bf144.3 &      \bf3.1 &    80.4      \\
\midrule
WCE                                     &    \bf35.8 &   22.7 &    \bf35.6 &    \bf2.7 &     \bf5.3 &    13.9 &   80.9 &    13.0 &   40.2      \\
WCE + ViLHub                            &    34.6 &   \bf20.6 &    33.3 &    5.2 &     4.7 &    \bf15.7 &   \bf73.2 &    \bf13.6 &   \bf39.6     \\
\midrule
FC                                      &    49.4 &   47.7 &    48.9 &    1.7 &    \bf13.4 &     6.1 &  604.6 &     1.5 &  141.6      \\
\midrule
DCPL$_\tau$~\cite{Kang2020Decoupling}     &    \bf49.3 &   48.1 &    \bf48.9 &    1.7 &    \bf13.3 &     6.1 &  606.6 &     1.5 &  141.1      \\
DCPL$_m$                                  &    45.9 &   25.8 &    46.0 &    \bf1.5 &    11.1 &     8.2 &  355.0 &     4.7 &  108.3      \\
DCPL$_m$ + ViLHub100k                     &     45.8 &    \bf24.5 &     39.9 &     3.7 &      9.5 &      \bf9.3 &   \bf336.7 &      \bf5.2 &    \bf66.7 \\

\bottomrule
\end{tabular}
}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{table*}


==> tables/gvqa_per_class_mean_analysis.tex <==
\begin{table*}[ht]
\caption{\label{tab:avg_per_class_performance} Average \textit{per class} performance}

\begin{center}
\begin{tabular}{c|ccccc|cccc}
Model & Acc & MR & GNews & VG & JCN & Acc &  MR & GNews & VG \\
\hline 
\hline
Baseline                 &15.30         &43.96  &0.406     &0.379   &0.242  &2.28                   &75.88  &0.398    &0.329  \\
FL ($\gamma=0.25$)  &14.61         &41.99  &0.407     &0.380   &0.238   &1.79                       &96.53  &0.394    &0.319  \\
FL ($\gamma=1$)     &15.05         &41.54  &0.406     &0.383   &0.241   &1.79                       &97.85  &0.392    &0.320  \\
FL ($\gamma=2$)     &14.89         &42.17  &0.409     &0.382   &0.242   &1.76                       &96.88  &0.390    &0.320  \\
FL ($\gamma=5$)     &15.34         &40.46    &0.413  &0.385      &0.243   &1.87                     &97.69  &0.393    &0.323  \\
FL ($\gamma=10$)    &15.26         &{\bf 39.73}   &{\bf 0.415}     &0.385   &0.242   &1.96          &96.00  &0.390    &0.324  \\
FL ($\gamma=50$)    &13.56         &41.01        &0.396          &0.370    &0.230   &1.77          &100.31  &0.380    &0.321  \\
Hubness                  &15.44         &43.39  &0.410     &0.383   &0.242   &{\bf 2.29}            &{\bf 74.60}  &0.400    &0.327    \\
Hubness 10K              &{\bf 15.72}   &43.06  &0.414     &{\bf 0.387}   & {\bf 0.245}   &2.18     &77.78  &{\bf 0.402}    &0.326  \\
Hubness 50K              &15.32         &43.27  &0.410     &0.383   &0.242   &2.24                  &76.39  &0.400    &{\bf 0.330}  \\
\hline 
\end{tabular}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{center}
\end{table*}





==> tables/gvqa_simple_mean_analysis.tex <==
\begin{table*}[ht]

\centering
\caption{\label{tab:overall_performance} Overall Average Performance Metrics}
\begin{tabular}{c|ccccc|cccc}
Model & Acc & MR & GNews & VG & JCN & Acc & MR & GNews & VG \\
\hline 
\hline
Baseline                &52.00	     &9.25	        &0.646          &0.669          &0.613       &48.85	    &1.12  & 0.914  &0.943    \\
FL ($\gamma=0.25$)   &{\bf 52.62} &8.86	        &{\bf 0.652}    &{\bf 0.676}    &{\bf 0.619}    &48.62	    &1.28   &0.913  &0.943    \\
FL ($\gamma=1$)      &52.35	     &8.82	        &0.649          &0.674          &0.617    &48.70	        &1.28   &0.913  &0.944    \\
FL ($\gamma=2$)      &52.06	     &{\bf 8.79}  	&0.647          &0.672          &0.615    &48.68	        &1.28   &0.913  &0.944    \\
FL ($\gamma=5$)      &51.34	     &8.57	        &0.643          &0.668          &0.610    &48.76	        &1.27   &0.914  &0.944    \\
FL ($\gamma=10$)     &50.13	     &8.90          &0.635          &0.660          &0.599    &48.52	        &1.27   &0.910  &0.941    \\
FL ($\gamma=50$)        &49.56	     &8.86	    &0.627          &0.654          &0.593    &48.27	        &1.34   &0.906  &0.938    \\
Hubness                 &51.65	     &9.42	        &0.643          &0.667          &0.611    &{\bf 49.00}	&{\bf 1.11}   &0.914  &0.944    \\
Hubness 10K             &51.95	     &9.37	        &0.646          &0.670          &0.613    &48.94	    &1.13   &{\bf 0.915}  &{\bf 0.945}    \\
Hubness 50K             &51.95	     &9.07	        &0.646          &0.668          &0.612    &48.93	    &1.12   &0.914  &0.944    \\
\hline 
\end{tabular}

\end{table*}

==> tables/many_median_few.tex <==
\begin{table*}[ht!]
\centering
\caption{\label{tab:many_medium_few} Performance on GQA}
\scalebox{0.8}
{
\begin{tabular}{l|cccc|cccc}
\toprule
{}              & \multicolumn{4}{c}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
\midrule
Model &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
Baseline~\cite{zhang2019large}            &    \bf70.5 &      36.2 &    3.5 &   51.9 &    \bf50.7 &       5.5 &    0.2 &   \bf49.7 \\  
Baseline + ViLHub 10k                     &    70.3 &      38.7 &    4.9 &   52.7 &    49.8 &       \bf9.5 &    \bf0.3 &   48.9 \\      
Baseline + ViLHub 50k                     &    69.8 &      41.4 &    7.6 &   53.5 &    49.0 &       8.4 &    0.2 &   48.1 \\         
Baseline + ViLHub 100k                    &    69.9 &      \bf41.9 &    \bf8.8 &   \bf53.8 &    48.8 &       7.2 &    0.1 &   47.9 \\     
\midrule
FL~\cite{lin2017focal}                    &    68.8 &      38.5 &    4.9 &   51.7 &    \bf50.4 &       4.6 &    0.0 &   \bf49.4 \\    
FL + ViLHub20k                          &    \bf69.8 &      \bf41.7 &    \bf8.1 &   \bf53.7 &    49.0 &       \bf7.0 &    \bf0.1 &   48.1 \\
\midrule
WCE                                      &    \bf39.3 &      36.5 &   16.2 &   \bf35.5 &    \bf35.9 &      29.0 &   14.3 &   \bf35.6 \\
WCE + ViLHub                            &    35.2 &      \bf39.5 &   \bf18.8 &   34.2 &    33.5 &      \bf31.3 &   \bf15.6 &   33.3 \\
\midrule
FC                                      &    71.6 &      26.9 &    0.1 &   49.5 &    50.0 &       0.0 &    0.0 &   49.0 \\
\midrule
DCPL$_\tau$~\cite{Kang2020Decoupling}   &    \bf71.4 &      27.0 &    0.1 &   \bf49.4 &    50.0 &       0.0 &    0.0 &   \bf48.9 \\
DCPL$_m$                                  &    61.0 &      34.1 &    4.4 &   45.9 &    46.7 &      17.9 &    0.4 &   46.0 \\           
DCPL$_m$ + ViLHub100k                     &    58.4 &      \bf38.1 &    \bf6.1 &   45.7 &    40.5 &      \bf21.3 &    \bf0.9 &   39.9 \\  
\bottomrule         
\end{tabular}
}
\end{table*}

==> tables/overall_word_similarity.tex <==
\begin{table*}[ht]
\caption{\label{tab:overrall_performance} Overall word similarity}

\begin{center}
\begin{tabular}{c|ccccc|c}
Model                   & sbj &     &     &      &     & rel  \\
                        & lch & lin & wup & path & w2v & w2v \\
\hline 
\hline
Baseline                &76.13   &79.49   &70.16   &63.54   &72.18  &51.82  \\
FL ($\gamma=2$)         &76.55   &79.88   &70.63   &64.00   &72.33   &51.70   \\
FL ($\gamma=5$)         &76.61   &79.92   &70.65   &64.06   &72.29   &51.75   \\
Fully Connected         &74.60   &78.22   &68.30   &61.26   &70.76   &51.40  \\
Decoupling              &72.66   &76.83   &65.27   &58.74   &67.51   &50.54  \\
Weighted CE             &69.59   &74.52   &60.76   &53.32   &62.81   &47.71   \\
\hline
FL ($\gamma=5$) + Hub20k &77.24    &80.41   &71.40   &65.15   &73.15   &51.59   \\
Hubness 10K             &76.69   &79.96   &70.82   &64.33   &72.71   &51.86    \\
Hubness 20K             &76.96   &80.19    &71.12   &64.72   &72.93   &51.72    \\
Hubness 50k             &77.30   &80.50   &71.51   &65.20   &73.23   &51.26    \\
Hubness 50k             &77.46   &80.64   &71.70   &65.48   &73.45   &51.14   \\
Weighted CE + Hub20k    &69.73   &74.92   &60.93   &53.06   &62.23   &46.86   \\

\hline 
\end{tabular}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{center}
\end{table*}

==> tables/per_class_word_similarity.tex <==
\begin{table}[ht]
\caption{\label{tab:overrall_performance} Per-class word similarity}

\begin{center}
\begin{tabular}{l|ccccc|c}
\toprule
 {}                     & \multicolumn{5}{|c|}{sbj/obj}  & rel  \\
\midrule
Model                   & lch & wup & lin & path & w2v & w2v \\
\midrule
Baseline~\cite{zhang2019large}          &     51.2 &     59.4 &     36.8 &      27.5 &     45.2 &     52.1 \\
FL~\cite{lin2017focal}                  &     51.8 &     60.0 &     37.5 &      28.3 &     45.7 &     51.7 \\
FC                                      &     48.9 &     57.1 &     33.8 &      24.5 &     43.3 &     51.6 \\
DCPL_\tau~\cite{Kang2020Decoupling}     &     49.0 &     57.3 &     33.9 &      24.5 &     43.2 &     51.6 \\
DCPL_m                                  &     49.1 &     57.4 &     34.1 &      25.8 &     43.0 &     50.5 \\
WCE                                     &     53.5 &     61.1 &     39.4 &      31.8 &     47.8 &     47.4 \\
ViLHub 100k                             &     53.4 &     61.3 &     39.5 &      30.6 &     47.1 &     51.3 \\
FL + ViLHub20k                          &     53.2 &     61.1 &     39.1 &      30.3 &     47.0 &     51.4 \\
WCE + ViLHub                            &     54.8 &     62.1 &     41.0 &      33.5 &     49.2 &     46.7 \\
\bottomrule
\end{tabular}

%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{center}
\end{table}


==> tables/pytorch_gvqa_overall_metrics.tex <==
\begin{table*}[ht]
\caption{\label{tab:overall_performance} Overall performance}

\begin{center}
\begin{tabular}{c|cc|cc|c}
Model                   & sbj &     & rel &     & triplet                   \\        
                        & acc & mr  & acc &  mr & acc                        \\       
\hline 
\hline
Baseline                &51.91   &5.91   &{\bf 49.96}   &{\bf 0.47}   &14.69 \\   
FL ($\gamma=2$)         &52.09   &6.10   &49.57   &0.50   &14.66              \\         
FL ($\gamma=5$)         &52.13   &6.05   &49.82   &0.48   &14.70              \\      
% FL ($\gamma=10$)        &   &   &   &   &   \\                                    
Fully Connected         &49.42   &18.94   &48.95   &0.67   &13.41              \\     
Decoupling              &45.99   &10.16   &45.99   &0.58   &11.08              \\     
WCE             &36.09   &8.98   &35.63   &1.07   &5.26                     \\
\hline
FL ($\gamma=5$) + Hub20k  &53.51   &5.47   &48.35   &2.14   &15.16              \\    
Hubness 10K             &52.77   &5.56   &49.10   &1.26   &14.94                 \\   
Hubness 20K             &53.20   &5.41   &48.98   &1.56   &15.08                  \\  
Hubness 50k             &53.73   &5.14   &48.08   &2.12   &15.18                  \\  
Hubness 100k            &{\bf 54.04}   &{\bf 5.12}   &47.88   &2.63   &{\bf 15.33} \\ 
WCE + Hub20k    &35.04   &8.17   &33.34   &2.07   &4.70                             \\
\hline 
\end{tabular}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{center}
\end{table*}








==> tables/pytorch_gvqa_per_class_mean_analysis.tex <==
% \begin{table*}[ht]
% \caption{\label{tab:avg_per_class_performance} Average \textit{per class} performance}

% \begin{center}
% \begin{tabular}{c|cc|cc}
% %                           SBJ                     REL
%                     & Sbj       &           & Rel       &       \\
% Model               & Acc       & MR        & Acc       &  MR   \\
% \hline 
% \hline
% Baseline            &8.66      &65.12       &2.76       &35.00  \\
% FL ($\gamma=0.25$)  &8.72      &66.44       &2.38       &38.31  \\
% FL ($\gamma=1$)     &8.80      &66.84       &2.57       &38.36  \\
% FL ($\gamma=2$)     &8.93      &65.71       &2.55       &38.10  \\
% FL ($\gamma=5$)     &9.20      &66.17       &2.87       &36.76  \\
% Hubness             &8.80      &70.37       &2.07       &47.67  \\
% %Hubness 10K         &15.72      &43.06       &2.18       &77.78  \\
% \hline 
% \end{tabular}
% %\bigskip
% %This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
% \end{center}
% \end{table*}



\begin{table*}[ht]
\caption{\label{tab:avg_per_class_performance} Average \textit{per class} performance}

\begin{center}
\begin{tabular}{c|cc|cc}
%                           SBJ                     REL
                    & Sbj       &           & Rel       &       \\
Model               & Acc       & MR        & Acc       &  MR   \\
\hline 
\hline
Baseline            &8.85      &77.84       &2.19       &37.81  \\
Hubness             &8.91      &78.12       &2.19       &37.94  \\
Hubness 10K         &9.97      &75.29       &2.35       &42.63  \\
FL ($\gamma=0.25$)  &8.64      &81.68       &1.98       &43.83  \\
FL ($\gamma=1$)     &8.70      &81.63       &2.00       &43.55  \\
FL ($\gamma=2$)     &8.89      &83.83       &2.01       &43.17  \\
FL ($\gamma=5$)     &9.15      &82.57       &2.10       &43.43  \\
FL ($\gamma=10$)     &9.51      &83.45       &2.20       &42.80  \\
\hline
\end{tabular}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{center}
\end{table*}


==> tables/pytorch_gvqa_per_class_metrics.tex <==
\begin{table*}[ht]
\caption{\label{tab:avg_per_class_performance} Average \textit{per class} performance}

\begin{center}
\begin{tabular}{c|cc|cc|c}
Model                   & sbj &     & rel &     & triplet   \\
                        & acc & mr  & acc &  mr & acc       \\
\hline 
\hline
Baseline                &8.48   &67.45   &2.82   &36.00   &1.01   \\
FL ($\gamma=2$)         &8.94   &65.90   &2.55   &38.10   &0.90   \\
FL ($\gamma=5$)         &9.24   &66.06   &2.87   &36.76   &1.04   \\
% FL ($\gamma=10$)        &   &   &   &   &   \\
Fully Connected         &6.13   &242.24   &1.54   &56.63   &0.48   \\
Decoupling              &8.27   &142.05   &4.74   &43.32   &1.35   \\
Weighted CE             &13.91   &32.16   &12.98   &16.07   &{\bf 2.48}   \\
\hline
FL ($\gamma=5$) + Hub20k  &10.99   &58.01   &2.61   &43.66   &0.93   \\
Hubness 10K             &9.25   &62.70   &2.93   &40.81   &0.99   \\
Hubness 20K             &9.91   &60.21   &2.86   &40.66   &0.99   \\
Hubness 50k             &10.77   &54.47   &3.29   &30.94   &1.19   \\
Hubness 100k            &11.29   &50.08   &3.17   &30.91   &1.18   \\
Weighted CE + Hub20k    &{\bf 15.72}   &{\bf 29.08}   &{\bf 13.59}   &{\bf 15.83}   &2.46   \\

\hline 
\end{tabular}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{center}
\end{table*}





==> tables/pytorch_gvqa_simple_mean_analysis.tex <==
% \begin{table*}[ht]

% \centering
% \caption{\label{tab:overall_performance} Overall Average Performance Metrics}
% \begin{tabular}{c|cc|cc}
% %                           SBJ                     REL
%                     & Sbj       &           & Rel       &       \\

% Model               & Acc       & MR        & Acc       &  MR   \\
% \hline 
% \hline
% Baseline            &51.64      &6.08       &50.03       &0.46  \\
% FL ($\gamma=0.25$)  &51.71      &6.23       &49.81       &0.51  \\
% FL ($\gamma=1$)     &51.83      &6.29       &49.90       &0.50  \\
% FL ($\gamma=2$)     &51.94      &6.19       &49.57       &0.50  \\
% FL ($\gamma=5$)     &51.94      &6.14       &49.82       &0.48  \\
% Hubness             &51.44      &8.30       &49.34       &1.32  \\
% %Hubness 10K         &15.72      &43.06       &2.18       &77.78  \\
% \hline 
% \end{tabular}

% \end{table*}


\begin{table*}[ht]

\centering
\caption{\label{tab:overall_performance} Overall Average Performance Metrics}
\begin{tabular}{c|cc|cc}
%                           SBJ                     REL
                    & Sbj       &           & Rel       &       \\

Model               & Acc       & MR        & Acc       &  MR   \\
\hline 
\hline
Baseline            &49.20      &10.15       &55.08       &2.85  \\
Hubness             &49.19      &10.22       &54.92       &2.88  \\
Hubness 10K         &50.74      &9.78      &55.06       &4.87  \\
FL ($\gamma=0.25$)  &49.10      &10.80       &52.65       &3.51  \\
FL ($\gamma=1$)     &49.10      &10.91       &53.08       &3.44  \\
FL ($\gamma=2$)     &49.49      &11.03       &53.25       &3.35  \\
FL ($\gamma=5$)     &49.40      &11.03       &53.87       &3.34  \\
FL ($\gamma=10$)     &49.12      &10.96       &53.72       &3.16  \\
\hline 
\end{tabular}

\end{table*}

==> tables/supp_mat_gvqa_per_class_mean.tex <==
% \begin{table*}[ht]
% \begin{center}
% \label{supp:gvqa_cm}
% \begin{tabular}{c||ccc|ccc|ccc}
% Model & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10\\
% \hline 
% \hline
% Baseline &15.6\pm0.2 &41.55\pm0.58 &53.49\pm0.39 &15.46\pm0.19 &41.38\pm0.45 &53.29\pm0.26 &2.29\pm0.06 &8.79\pm0.2 &14.15\pm0.45 \\
% Hubness  &15.67\pm0.06 &41.89\pm0.01 &54.25\pm0.56 &15.44\pm0.01 &41.64\pm0.22 &53.97\pm0.42 &2.27\pm0.07 &8.78\pm0.09 &14.28\pm0.14 \\
% Hubness 10K &15.56\pm0.25 &41.5\pm0.01 &53.64\pm0.16 &15.37\pm0.27 &41.20\pm0.17 &53.35\pm0.18 &2.23\pm0.04 &8.66\pm0.3 &14.15\pm0.61 \\
% \hline 
% \end{tabular}
% \caption{\label{tab:avg_per_class_performance} \textbf{Average \textit{per class} performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1,5 and 10 model predictions. The results are averages based on 4 random-seeds controlling the network-initialization and the data-set splits.}
% \end{center}
% \end{table*}



\begin{table*}[ht]
\begin{center}
\label{supp:gvqa_cm}
\begin{tabular}{c||cc|cc|cc}
Model & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5 \\
\hline 
\hli
Baseline    &15.6\pm0.2     &41.55\pm0.58  &{\bf 15.46}\pm0.19 &41.38\pm0.45 &{\bf 2.29}\pm0.06 &{\bf 8.79}\pm0.2  \\
Hubness     &{\bf 15.67}\pm0.06   &{\bf 41.89}\pm0.01  &15.44\pm0.01 &{\bf 41.64}\pm0.22 &2.27\pm0.07 &8.78\pm0.09 \\
Hubness 10K &15.56\pm0.25   &41.5\pm0.01   &15.37\pm0.27 &41.20\pm0.17 &2.23\pm0.04 &8.66\pm0.3  \\
\hline 
\end{tabular}
\caption{\label{tab:avg_per_class_performance} \textbf{Average \textit{per class} performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1, and 5 model predictions. The results are averages based on several random-seeds controlling the network-initialization and the data-set splits.}
\end{center}
\end{table*}





==> tables/supp_mat_gvqa_simple_mean.tex <==
% \begin{table*}[ht]
% \begin{center}
% \label{supp:vgqa_sm}
% \begin{tabular}{c||ccc|ccc|ccc}
% Model & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10\\
% \hline 
% \hline
% Baseline &52.08\pm0.28 &81.17\pm0.27 &87.52\pm0.28 &51.64\pm0.28 &80.93\pm0.26 &87.35\pm0.25 &48.87\pm0.06 &97.26\pm0.06 &98.47\pm0.03 \\
% Hubness  &51.89\pm0.15 &80.97\pm0.41 &87.35\pm0.44 &51.46\pm0.16 &80.73\pm0.4 &87.2\pm0.41 &48.92\pm0.06 &97.22\pm0.06 &98.47\pm0.03  \\
% Hubness 10K &52.02\pm0.28 &81.04\pm0.27 &87.46\pm0.22 &51.59\pm0.29 &80.82\pm0.28 &87.31\pm0.22 &48.88\pm0.06 &97.24\pm0.04 &98.47\pm0.01 \\
% \hline 
% \end{tabular}
% \caption{\label{tab:avg_per_class_performance} \textbf{Average performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1,5 and 10 model predictions. The results are averages based on 4 random-seeds controlling the network-initialization and the data-set splits.}
% \end{center}
% \end{table*}

\begin{table*}[ht]
\begin{center}
\label{supp:vgqa_sm}
\begin{tabular}{c||cc|cc|cc}
Model & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5\\
\hline 
\hline
Baseline    &{\bf 52.08}\pm0.28   &{\bf 81.17}\pm0.27   &{\bf 51.64}\pm0.28   &{\bf 80.93}\pm0.26    &48.87\pm0.06 &{\bf 97.26}\pm0.06 \\
Hubness     &51.89\pm0.15   &80.97\pm0.41   &51.46\pm0.16   &80.73\pm0.4     &{\bf 48.92}\pm0.06 &97.22\pm0.06  \\
Hubness 10K &52.02\pm0.28   &81.04\pm0.27   &51.59\pm0.29   &80.82\pm0.28    &48.88\pm0.06 &97.24\pm0.04 \\
\hlin
\end{tabular}
\caption{\label{tab:avg_per_class_performance} \textbf{Average performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1, and 5 model predictions. The results are averages based on several random-seeds controlling the network-initialization and the data-set splits.}
\end{center}
\end{table*}





==> tables/supp_mat_vg_per_class_mean.tex <==
% \begin{table*}[ht]
% \begin{center}
% \label{supp:vg_cm}
% \begin{tabular}{c||ccc|ccc|ccc}
% Model & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10\\
% \hline 
% \hline
% Baseline &5.71\pm0.18 &18.12\pm0.51 &25.69\pm1.04 &5.27\pm0.27 &16.75\pm0.63 &23.41\pm0.71 &0.37\pm0.02 &2.044\pm0.05 &3.78\pm0.07 \\
% Hubness  &5.79\pm0.28 &18.25\pm0.69 &25.54\pm1.19 &5.35\pm0.25 &17.01\pm0.79 &23.62\pm0.90 &0.38\pm0.02 &2.04\pm0.12 &3.69\pm0.04 \\
% Hubness 10K &5.84\pm0.12 &18.17\pm0.38 &25.78\pm0.39 &5.45\pm0.16 &17.05\pm0.22 &23.89\pm0.56 &0.37\pm0.01 &2.09\pm0.04 &3.77\pm0.13 \\
% \hline 
% \end{tabular}
% \caption{\label{tab:avg_per_class_performance} \textbf{Average \textit{per class} performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1,5 and 10 model predictions. The results are averages based on 4 random-seeds controlling the network-initialization and the data-set splits.}
% \end{center}
% \end{table*}

\begin{table*}[ht]
\begin{center}
\label{supp:vg_cm}
\begin{tabular}{c||cc|cc|cc}
Model & Top-1 & Top-5  & Top-1 & Top-5  & Top-1 & Top-5 \\
\hline 
\hline
Baseline        &5.71\pm0.18 &18.12\pm0.51  &5.27\pm0.27 &16.75\pm0.63  &0.37\pm0.02 &2.044\pm0.05  \\
Hubness         &5.79\pm0.28 &{\bf 18.25}\pm0.69  &5.35\pm0.25 &17.01\pm0.79  &{\bf 0.38}\pm0.02 &2.04\pm0.12   \\
Hubness 10K     &{\bf 5.84}\pm0.12 &18.17\pm0.38  &{\bf 5.45}\pm0.16 &{\bf 17.05}\pm0.22  &0.37\pm0.01 &{\bf 2.09}\pm0.04   \\
\hline 
\end{tabular}
\caption{\label{tab:avg_per_class_performance} \textbf{Average \textit{per class} performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1, and 5 model predictions. The results are averages based on several random-seeds controlling the network-initialization and the data-set splits.}
\end{center}
\end{table*}

==> tables/supp_mat_vg_simple_mean.tex.tex <==
% \begin{table*}[ht]
% \begin{center}
% \label{supp:vg_sm}
% \begin{tabular}{c||ccc|ccc|ccc}
% Model & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10 & Top-1 & Top-5 & Top-10\\
% \hline 
% \hline
% Baseline &50.89\pm0.49 &77.06\pm0.4 &82.91\pm0.44 &48.24\pm0.38 &74.15\pm0.4 &80.5\pm0.28 &53.08\pm0.29 &79.67\pm0.1 &85.65\pm0.07 \\
% Hubness  &50.71\pm0.18 &76.9\pm0.23 &82.62\pm0.25 &48.3\pm0.26 &74.1\pm0.2 &80.32\pm0.2 &52.68\pm0.23 &79.62\pm0.1 &85.58\pm0.07 \\
% Hubness 10K &51.04\pm0.2 &77.31\pm0.29 &83.07\pm0.29 &48.71\pm0.2 &74.59\pm0.29 &80.89\pm0.27 &52.88\pm0.43 &79.68\pm0.16 &85.7\pm0.075 \\
% \hline 
% \end{tabular}
% \caption{\label{tab:avg_per_class_performance} \textbf{Average performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1,5 and 10 model predictions. The results are averages based on 4 random-seeds controlling the network-initialization and the data-set splits.}
% \end{center}
% \end{table*}



\begin{table*}[ht]
\begin{center}
\label{supp:vg_sm}
\begin{tabular}{c||cc|cc|cc}
Model & Top-1 & Top-5 & Top-1 & Top-5 & Top-1 & Top-5\\
\hline 
\hline
Baseline    &50.89\pm0.49   &77.06\pm0.4    &48.24\pm0.38   &74.15\pm0.4    &{\bf 53.08}\pm0.29 &79.67\pm0.1  \\
Hubness     &50.71\pm0.18   &76.9\pm0.23    &48.3\pm0.26    &74.1\pm0.2     &52.68\pm0.23 &79.62\pm0.1  \\
Hubness 10K &{\bf 51.04}\pm0.2    &{\bf 77.31}\pm0.29   &{\bf 48.71}\pm0.2    &{\bf 74.59}\pm0.29   &52.88\pm0.43 &{\bf 79.68}\pm0.16 \\
\hline 
\end{tabular}
\caption{\label{tab:avg_per_class_performance} \textbf{Average performance of different methods.} The numbers are the obtained accuracy for  \textit{object} types (left-most panel),  \textit{subjects} (middle panel) and   \textit{relation} types (right-most panel). Here, we use the accuracy metric for the top-1,and 5model predictions. The results are averages based on several random-seeds controlling the network-initialization and the data-set splits.}
\end{center}
\end{table*}



==> tables/vg8k_many_median_few_pc.tex <==
\begin{table*}[ht!]
\centering
\caption{\label{tab:vg_many_medium_few} Performance on VG}
\scalebox{0.8}
{
\begin{tabular}{l|cccc|cccc}
\toprule
{}              & \multicolumn{4}{|c|}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
{}                                         &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
Baseline~\cite{zhang2019large}             &        57.0 &           8.5 &        0.0 &        4.1 &       12.8 &          0.6 &       0.0 &       0.7 \\
Baseline + ViLHub 10K                      &        58.2 &           9.7 &        0.0 &        4.4 &       16.2 &          0.7 &       0.0 &       0.9 \\
Baseline + ViLHub 100K                     &        60.2 &          14.8 &        0.2 &        5.4 &       16.4 &          0.1 &       0.0 &       0.8 \\
\midrule
WCE                                        &        51.5 &          22.0 &        2.0 &        7.5 &       26.6 &         11.6 &       1.2 &       4.1 \\
WCE + ViLHub                               &        50.5 &          22.8 &        2.5 &        7.9 &       26.8 &         11.7 &       1.0 &       3.9 \\
\midrule
FL~\cite{lin2017focal}                     &        56.9 &          12.2 &        0.1 &        4.7 &       13.0 &          0.3 &       0.0 &       0.7 \\
\midrule
FC                                         &       55.5 &          5.8 &       0.3 &       3.9 &       11.3 &          4.9 &       0.6 &       1.7 \\
DCPL$_m$~\cite{Kang2020Decoupling}         &        52.6 &           4.3 &        0.0 &        3.3 &       23.7 &          0.9 &       0.0 &       1.3 \\
\bottomrule
\end{tabular}
}
\end{table*}


==> tables/vg8k_many_median_few_pc_syn.tex <==
\begin{table}[t!]
\parbox{.49\linewidth}{
\centering
\caption{\label{tab:vg8k_many_median_few_pc_syn} Performance on VG8K based on Synsets}
\scalebox{0.5}{
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
{}              & \multicolumn{4}{|c|}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
{}                                         &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
~\cite{zhang2019large}                      &        58.3 &          13.3 &        8.3 &       11.3 &       24.2 &         14.4 &      14.1 &      14.6 \\
~\cite{zhang2019large} + ViLHub 10K         &        59.4 &          14.9 &        8.5 &       11.7 &       27.5 &         14.7 &      15.1 &      15.7 \\
~\cite{zhang2019large} + ViLHub 100K        &        61.4 &          20.8 &        9.5 &       13.3 &       27.9 &         14.2 &      13.9 &      14.6 \\
\Delta                                      &         \bf+1.1 &           \bf+1.3 &        \bf+0.2 &        \bf+0.4 &        \bf+3.3 &          \bf+0.9 &       \bf+0.9 &       \bf+1.1 \\
\midrule
WCE                                         &        52.8 &          27.2 &       10.8 &       14.5 &       35.5 &         24.7 &      15.2 &      17.2 \\
WCE + ViLHub                                &        52.0 &          27.9 &       11.1 &       14.8 &       35.2 &         24.6 &      15.3 &      17.2 \\
\Delta                                      &        \bf-0.8 &           \bf+0.7 &        \bf+0.3 &        \bf+0.3 &       \bf-0.3 &          \bf+0.1 &       \bf+0.1 &       \bf0.0 \\
\midrule
FL~\cite{lin2017focal}                      &        58.1 &          17.8 &        8.8 &       12.1 &       24.5 &         14.0 &      14.2 &      14.7 \\
\midrule
FC                                          &        64.0 &           7.5 &        8.8 &       11.4 &       21.6 &         11.0 &      11.6 &      12.0 \\
DCPL$_m$~\cite{Kang2020Decoupling}          &        53.8 &           7.4 &        7.6 &        9.9 &       34.3 &         14.2 &      13.2 &      14.4 \\
\bottomrule
\end{tabular}
}
}
\end{table}

\begin{table*}
\parbox{.57\linewidth}{
\centering
\resizebox{.56\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
Split-Mode & Easy & Hard & Easy & Hard &  & Easy & Hard & Easy & Hard \\ \midrule
WAC-Linear \cite{elhoseiny2013write} & 27.0 & 5.0 & -- & -- &  & 23.9 & 4.9 & 23.5 & -- \\
WAC-Kernel \cite{elhoseiny2016write} & 33.5 & 7.7 & 11.4 & 6.0 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
ESZSL \cite{romera2015embarrassingly} & 28.5 & 7.4 & 24.3 & 6.3 &  & 18.5 & 4.5 & 9.2 & 2.9 \\
ZSLNS \cite{Qiao2016} & 29.1 & 7.3 & 24.5 & 6.8 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 & 18.4 & 3.8 &  & 13.1 & 4.0 & 2.7 & 3.5 \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 & 5.9 & -- & -- &  & 1.7 & 1.0 & 0.1 & --\\
ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2 & 9.7 &30.3 & 8.1 &  & 30.4 & 6.1 & 12.6 & 3.5 \\ \hline
FeatGen~\cite{xian2018feature} &  43.9 & 9.8 &36.2 & 8.7 &  & 34.1 & 7.4 & 21.3 & 5.6 \\
FeatGen\cite{xian2018feature}+ \textbf{CIZSL} &  44.2\mathcolor{blue}{\mathbf{ $^{+0.3}$}}  & 12.1 \mathcolor{blue}{\mathbf{ $^{+2.3}$}}  & 36.3 \mathcolor{blue}{\mathbf{ $^{+0.1}$}} & \textbf{9.8} \mathcolor{blue}{\mathbf{ $^{+1.1}$}} &  & 37.4 \mathcolor{blue}{\mathbf{ $^{+2.7}$}} & 9.8\mathcolor{blue}{\mathbf{ $^{+2.4}$}} & 24.7\mathcolor{blue}{\mathbf{ $^{+3.4}$}} & 6.2 \mathcolor{blue}{\mathbf{ $^{+0.6}$}} \\  \hline
GAZSL~\cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\    \midrule
GAZSL~\cite{Elhoseiny_2018_CVPR} + \textbf{CIZSL} &  \textbf{44.6} \mathcolor{blue}{\mathbf{ $^{+0.9}$}} & \textbf{14.4} \mathcolor{blue}{\mathbf{ $^{+4.1}$}} & \textbf{36.6} \mathcolor{blue}{\mathbf{ $^{+1.0}$}} & 9.3 \mathcolor{blue}{\mathbf{ $^{+0.7}$}} &  & \textbf{39.2}\mathcolor{blue}{\mathbf{ $^{+3.8}$}} & \textbf{11.9}\mathcolor{blue}{\mathbf{ $^{+3.2}$}} & \textbf{24.5}\mathcolor{blue}{\mathbf{ $^{+4.1}$}} & \textbf{6.4}\mathcolor{blue}{\mathbf{ $^{+0.6}$}}\\ \bottomrule
\end{tabular}%
}
\caption{Zero-Shot Recognition on class-level textual description from \textbf{CUB} and \textbf{NAB} datasets with two-split setting.}
\label{tb:nab_cub}
\vspace{-1.67ex}
}
\hfill
\parbox{.4\linewidth}{
\centering
\resizebox{.4\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
 & \multicolumn{3}{c}{Top-1 Accuracy(\%)} &  & \multicolumn{3}{c}{Seen-Unseen H} \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
 & AwA2 & aPY & SUN &  & AwA2 & aPY & SUN \\ \midrule
DAP~\cite{Lampert2014} & 46.1 & 33.8 & 39.9 &  & -- & 9.0 & 7.2 \\
SSE~\cite{zhang2015zero} & 61.0 & 34.0 & 51.5 &  & 14.8 & 0.4 & 4.0 \\
SJE~\cite{akata2015evaluation} & 61.9 & 35.2 & 53.7 &  & 14.4 & 6.9 & 19.8 \\
LATEM~\cite{xian2016latent} & 55.8 & 35.2 & 55.3 &  & 20.0 & 0.2 & 19.5 \\
ESZSL~\cite{romera2015embarrassingly} & 58.6 & 38.3 & 54.5 &  & 11.0 & 4.6 & 15.8 \\
ALE~\cite{akata2016label} & 62.5 & 39.7 & 58.1 &  & 23.9 & 8.7 & 26.3 \\
CONSE~\cite{norouzi2013zero} & 44.5 & 26.9 & 38.8 &  & 1.0 & -- & 11.6 \\
SYNC~\cite{changpinyo2016synthesized} & 46.6 & 23.9 & 56.3 &  & 18.0 & 13.3 & 13.4 \\
SAE~\cite{kodirov2017semantic} & 54.1 & 8.3 & 40.3 &  & 2.2 & 0.9 & 11.8 \\
DEM~\cite{zhang2016learning} & 67.1 & 35.0 & 61.9 &  & 25.1 & 19.4 & 25.6 \\
DEVISE~\cite{frome2013devise} & 59.7 & 39.8 & 56.5 &  & \textbf{27.8} & 9.2 & 20.9 \\  \hline
GAZSL~\cite{Elhoseiny_2018_CVPR} & 58.9 & 41.1 & 61.3 &  & 15.4 & 24.0 & 26.7 \\ 
GAZSL~\cite{Elhoseiny_2018_CVPR} + \textbf{CIZSL} & \textbf{67.8} \mathcolor{blue}{\mathbf{ $^{+8.9}$}} & {42.1} \mathcolor{blue}{\mathbf{ $^{+1.0}$}} & {63.7} \mathcolor{blue}{\mathbf{ $^{+2.4}$}} &  & 24.6 \mathcolor{blue}{\mathbf{ $^{+9.2}$}} & {25.7} \mathcolor{blue}{\mathbf{ $^{+1.7}$}} & \textbf{27.8} \mathcolor{blue}{\mathbf{ $^{+1.1}$}}  \\
\hline \hline
FeatGen~\cite{xian2018feature} & 54.3 & 42.6 & 60.8 &  & 17.6 & 21.4 & 24.9 \\
FeatGen~\cite{xian2018feature} + \textbf{CIZSL} & 60.1\mathcolor{blue}{\mathbf{ $^{+5.8}$}}  & 43.8\mathcolor{blue}{\mathbf{ $^{+1.2}$}} & 59.4\mathcolor{red}{\mathbf{ $^{-0.6}$}} &  & 19.1\mathcolor{blue}{\mathbf{ $^{+1.5}$}}  & 24.0 \mathcolor{blue}{\mathbf{ $^{+2.6}$}} & 26.5 \mathcolor{blue}{\mathbf{ $^{+1.6}$}} \\
\midrule
cycle-(U)WGAN~\cite{felix2018multi} & 56.2 & 44.6 & 60.3 &  & 19.2 & 23.6 & 24.4 \\
cycle-(U)WGAN~\cite{felix2018multi} + \textbf{CIZSL} & 63.6 \mathcolor{blue}{\mathbf{ $^{+7.4}$}}  & \textbf{45.1} \mathcolor{blue}{\mathbf{ $^{+0.5}$}}  & \textbf{64.2} \mathcolor{blue}{\mathbf{ $^{+3.9}$}}   &  & 23.9 \mathcolor{blue}{\mathbf{ $^{+4.7}$}}   & \textbf{26.2} \mathcolor{blue}{\mathbf{ $^{+2.6}$}}   & 27.6 \mathcolor{blue}{\mathbf{ $^{+3.2}$}}  \\
\bottomrule
\end{tabular}%
}
\caption{Zero-Shot Recognition on class-level attributes of \textbf{AwA2}, \textbf{aPY} and \textbf{SUN} datasets.}
\label{tb:awa2_apy_sun}
}
\vspace{-2.0ex}
\end{table*}

\begin{table*}
\vspace{-4mm}
\parbox{.60\linewidth}{
\centering
\resizebox{.60\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
Split-Mode & Easy & Hard & Easy & Hard &  & Easy & Hard & Easy & Hard \\ \midrule
\textbf{CIZSL SM-Entropy (ours final)} & \textbf{44.6} & \textbf{14.4} & 36.5 & \textbf{9.3} &  & \textbf{39.2} & \textbf{11.9} & \textbf{24.5} & \textbf{6.4} \\ \hline 
CIZSL SM-Entropy (replace $2^{nd}$ term in Eq~\ref{eq_lgc} by Classifying $t^h$ as new class) & 43.2 & 11.31 & 35.6 & 8.5 &  &38.3 & 9.5 & 21.6 & 5.6\\ 
CIZSL SM-Entropy (minus  $1^{st}$ term in Eq~\ref{eq_lgc}) & 43.4 & 10.1 & 35.2 & 8.3 &  & 35.0 & 8.2 & 20.1  & 5.4\\  
CIZSL SM-Entropy: (minus  $2^{nd}$ term in Eq~\ref{eq_lgc}) & 41.7 & 11.2 & 33.4 & 8.1 &  & 33.3 & 10.1 & 21.3 & 5.1\\
\hline 
CIZSL Bachatera-Entropy ($\gamma=0.5,\beta =0.5$) & 44.1 & 13.7 & 35.9 & 8.9 &  & 38.9 & 10.3 & 24.3 & 6.2\\
CIZSL Renyi-Entropy ($\beta \to 1$) &  44.1 & 13.3 & 35.8 & 8.8 &  & 38.6 & 10.3 & 23.7 & 6.3\\	
CIZSL KL-Entropy ($\gamma \to 1,\beta \to 1$)	&  44.5 & 14.2 & 36.3 & 8.9 &  & 38.9 & 11.6 & 24.3 & 6.2\\
CIZSL Tsallis-Entropy ($\beta = \gamma$) & 44.1 & 13.8 & \textbf{36.7} & 8.9 &  & 38.9 & 11.3 & 24.5 & 6.3  \\	  \hline
CIZSL SM-Entropy: (minus  $1^{st}$ and $2^{nd}$ terms in Eq~\ref{eq_lgc})= GAZSL~\cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\ 
\bottomrule
\end{tabular}%
}
\caption{Ablation Study using Zero-Shot recognition on \textbf{CUB} \& \textbf{NAB} datasets with two split settings each. CIZSL is GAZSL~\cite{Elhoseiny_2018_CVPR}+ our loss}
\label{tb:nab_cub_ablation}
}
\hfill
\parbox{.38\linewidth}{
\centering
\includegraphics[width=0.30\textwidth, height=3.62cm]{figures/ParakeetAuklet_vs_CrestedAukletAUC_final}
		\vspace{-3mm}
\captionof{figure}{Seen Unseen Curve for Parakeet Auklet (Seen,  y-axis) vs Crested Auklet (Unseen, x-axis) for GAZSL[57] and     GAZSL[57]+ CIZSL.}
\label{fig_auklet}
}
\vspace{-3.67ex}
\end{table*}

==> tables/vg8k_triplet.tex <==
\begin{table}
\centering
\caption{\label{tab:vg8k_triplets}Triplet Scores on VG8K using Synsets}
\scalebox{0.7}
{
\begin{tabular}{lrrrr}
\toprule
{} &  many &  median &  few &  all \\
\midrule
\cite{zhang2019large}                   &  24.0 &    10.1 &  3.1 &  5.2 \\
\cite{zhang2019large} + ViLHub 20k      &  21.6 &     7.3 &  4.3 &  5.6 \\
\Delta                                  &   \bf+0.8 &     \bf+0.5 &  \bf+0.2 &  \bf+0.3 \\
\midrule
WCE                                     &  10.1 &     4.4 &  2.8 &  3.4 \\
WCE + ViLHub                            &   9.2 &     4.1 &  2.7 &  3.3 \\
\Delta                                  &  \bf-0.9 &    \bf-0.3 & \bf-0.1 & \bf-0.1 \\
\midrule
FL~\cite{lin2017focal}                  &  15.1 &     6.1 &  4.0 &  4.9 \\
DCPL~\cite{Kang2020Decoupling}          &  14.5 &     5.5 &  2.8 &  3.8 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/vg_combined_metrics.tex <==
\begin{table*}[ht!]
\centering
% \vspace{-2mm}
\caption{\label{tab:vg_combined_performance} Performance on Visual Genome}
\scalebox{0.8}
{
\begin{tabular}{l|cc|cc|c|cc|cc}
\toprule
 {}                             &      \multicolumn{5}{|c|}{Overall}                        & \multicolumn{4}{|c}{Per-class} \\
\midrule
 {}                             & \multicolumn{2}{|c|}{sbj/obj} & \multicolumn{2}{|c|}{rel} & triplet  & \multicolumn{2}{|c|}{sbj/obj} & \multicolumn{2}{|c}{rel}  \\
\midrule
Model                                       &    acc    &    mr  &    acc &      mr &       acc        & acc &  mr    &     acc &     mr  \\ 
\midrule
Baseline~\cite{zhang2019large}                      &    47.4 &   53.6 &    \bf54.0 &   \bf20.5 &    14.2 &     4.2 &   502.7 &     0.7 &  \bf414.1     \\
Baseline + ViLHub 10K                             &     48.2 &    53.7 &     52.8 &    22.0 &     14.5 &      4.4 &   502.0 &      \bf0.9 &   417.5     \\
Baseline + ViLHub 100K                             & \bf49.5 &    \bf49.0 &     51.3 &    34.4 &     \bf15.4 &      \bf5.4 &   \bf455.0 &      0.8 &   445.6  \\
\midrule
WCE                                         &    \bf40.0 &   \bf47.6 &    \bf23.8 &   29.9 &     \bf5.3 &     7.5 &   238.0 &     \bf4.1 &  250.6     \\
WCE + ViLHub                                    &    38.8 &   49.0 &    23.4 &   \bf29.4 &     5.0 &     \bf8.0 &   \bf228.5 &     3.92 &  \bf235.7  \\
\midrule
FL~\cite{lin2017focal}         &    45.3 &   62.3 &    50.3 &   25.4 &    12.0 &     4.8 &   575.3 &     0.7 &  475.4    \\
\midrule
FC                                          &    44.5 &  171.2 &    51.3 &   37.0 &    11.0 &     4.1 &  1334.1 &     0.5 &  660.0     \\
DCPL$_m$~\cite{Kang2020Decoupling}             &    43.1 &  128.0 &    42.6 &   30.5 &     9.5 &     3.3 &  1308.3 &     1.3 &  710.8    \\

\bottomrule
\end{tabular}
}
%\bigskip
%This table shows the performance of the models tested averaged over the classes, where all classes are weighted equally. This helps show any improvement on low frequency classes
\end{table*}







==> tables/vg_many_medium_few.tex <==
\begin{table}[ht!]
\centering
\caption{\label{tab:vg_many_medium_few} Performance on VG}
\scalebox{0.8}
{
\begin{tabular}{l|cccc|cccc}
\toprule
{}              & \multicolumn{4}{|c|}{sbj/obj} & \multicolumn{4}{|c}{rel} \\
{}                                          &  many &  medium &  few &  all &  many &  medium &  few &  all \\
\midrule
Baseline~\cite{zhang2019large}            &    65.5 &      16.6 &    0.3 &   46.8 &    \bf58.9 &       1.8 &    0.0 &   \bf54.0 \\
Baseline + ViLHub 10K                      &    \bf66.2 &      18.4 &    0.4 &   47.6 &    57.6 &       \bf2.0 &    0.0 &   52.8 \\
Baseline + ViLHub 100K                     &    65.7 &      \bf24.2 &    \bf1.3 &   \bf48.4 &    56.0 &       0.2 &    0.0 &   51.3 \\
\midrule
WCE                                        &    46.7 &      29.7 &    5.4 &   37.3 &    \bf25.1 &      \bf16.7 &    \bf3.3 &   23.8 \\
WCE + ViLHub                               &    44.3 &      \bf30.3 &    \bf6.1 &   36.0 &    24.6 &      16.5 &    \bf3.3 &   23.4 \\
\midrule
FL~\cite{lin2017focal}                     &    59.8 &      22.7 &    0.8 &   44.2 &    54.9 &       1.1 &    0.0 &   50.3 \\
\midrule
FC                                         &    68.1 &      13.2 &    0.0 &   43.1 &    57.7 &       0.0 &    0.0 &   51.3 \\
DCPL$_m$~\cite{Kang2020Decoupling}         &    60.9 &       9.6 &    0.0 &   42.4 &    46.4 &       2.3 &    0.0 &   42.6 \\
\bottomrule
\end{tabular}
}
\end{table}




